Verifying Quantum Circuits with Level-Synchronized Tree Automata (Technical Report)

We present a new method for the verification of quantum circuits based on a novel symbolic representation of sets of quantum states using level-synchronized tree automata (LSTAs). LSTAs extend classical tree automata by labeling each transition with a set of choices, which are then used to synchronize subtrees of an accepted tree. Compared to the traditional tree automata, LSTAs have an incomparable expressive power while maintaining important properties, such as closure under union and intersection, and decidable language emptiness and inclusion. We have developed an efficient and fully automated symbolic verification algorithm for quantum circuits based on LSTAs. The complexity of supported gate operations is at most quadratic, dramatically improving the exponential worst-case complexity of an earlier tree automata-based approach. Furthermore, we show that LSTAs are a promising model for parameterized verification, i.e., verifying the correctness of families of circuits with the same structure for any number of qubits involved, which principally lies beyond the capabilities of previous automated approaches. We implemented this method as a C++ tool and compared it with three symbolic quantum circuit verifiers and two simulators on several benchmark examples. The results show that our approach can solve problems with sizes orders of magnitude larger than the state of the art.

==> hidden_exp.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|}\hline
        \# of qubits & Running Time\\\hline
        $2^4=16$ & 0.095s -> 0.074s\\\hline
        $2^5=32$ & 0.462s -> 0.363s\\\hline
        $2^6=64$ & 2.930s -> 2.632s\\\hline
        $2^7=128$ & 22.121s -> 25.955s\\\hline
        $2^8=256$ & 2m53.297s -> 2m59.804s\\\hline
        $2^9=512$ & 25m14.131s\\\hline
    \end{tabular}
    \caption{Do H$^2$ with CTA.}
    \label{tab:h2}
\end{table}

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|}\hline
        \# of qubits & Running Time\\\hline
        $8$ & 0.293s\\\hline
        $9$ & 1.005s\\\hline
        $10$ & 4.137s\\\hline
        $11$ & 15.609s\\\hline
        $12$ & 1m19.134s\\\hline
        $13$ & 4m22.705s\\\hline
        $14$ & 18m20.955s\\\hline
        $15$ & 81m53.675s\\\hline
    \end{tabular}
    \caption{Do H$^2$ with TA.}
    \label{tab:h2}
\end{table}

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|}\hline
       n & G & sB & sA & tB & tA & time & x\\\hline
       8 & 16 & 17 & 47 & 25 & 32 & 0.0s & 0.0s\\\hline
       9 & 18 & 19 & 53 & 28 & 36 & 0.0s & 0.0s\\\hline
       10 & 20 & 21 & 59 & 31 & 40 & 0.0s & 0.0s\\\hline
       11 & 22 & 23 & 65 & 34 & 44 & 0.0s & 0.0s\\\hline
    \end{tabular}
    \caption{Do H2 with all-sim-reduce CTA.}
    % \label{tab:h3}
\end{table}

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|}\hline
       n & G & sB & sA & tB & tA & time & x\\\hline
       8 & 16 & 17 & 1035 & 25 & 519 & 1.0s & 0.0s\\\hline
       9 & 18 & 19 & 2061 & 28 & 1032 & 4.2s & 0.0s\\\hline
       10 & 20 & 21 & 4111 & 31 & 2057 & 21s & 0.0s\\\hline
       11 & 22 & 23 & 8209 & 34 & 4106 & 3m9s & 0.0s\\\hline
    \end{tabular}
    \caption{Do H2 with all-sim-reduce TA.}
    % \label{tab:h3}
\end{table}

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|}\hline
       n & G & sB & sA & tB & tA & time & x\\\hline
       99 & 297 & 199 & 593 & 298 & 593 & 10s & 0.0s\\\hline
    \end{tabular}
    \caption{Do HXH with CTA.}
    \label{tab:h3}
\end{table}

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|}\hline
       n & G & sB & sA & tB & tA & time & x\\\hline
       9 & 27 & 19 & 1032 & 28 & 1543 & 0.9s & 0.0s\\\hline
       10 & 30 & 21 & 2057 & 31 & 3080 & 3.6s & 0.0s\\\hline
       11 & 33 & 23 & 4106 & 34 & 6153 & 14s & 0.0s\\\hline
       12 & 36 & 25 & 8203 & 37 & 12298 & 1m0s & 0.0s\\\hline
       13 & 39 & 27 & 16396 & 40 & 24587 & 4m11s & 0.0s\\\hline
    \end{tabular}
    \caption{Do HXH with TA.}
    \label{tab:h4}
\end{table}

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|}\hline
       n & G & sB & sA & tB & tA & time & x\\\hline
       9 & 27 & 19 & 53 & 28 & 53 & 0.0s & 0.0s\\\hline
       10 & 30 & 21 & 59 & 31 & 59 & 0.0s & 0.0s\\\hline
       11 & 33 & 23 & 65 & 34 & 65 & 0.0s & 0.0s\\\hline
       99 & 297 & 199 & 593 & 298 & 593 & 12s & 0.0s\\\hline
    \end{tabular}
    \caption{Do HXH with all-sim-reduce CTA.}
    % \label{tab:h4}
\end{table}

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|}\hline
       n & G & sB & sA & tB & tA & time & x\\\hline
       9 & 27 & 19 & 2061 & 28 & 1543 & 4.3s & 0.0s\\\hline
       10 & 30 & 21 & 4111 & 31 & 3080 & 30s & 0.0s\\\hline
       11 & 33 & 23 & 8209 & 34 & 6153 & 3m53s & 0.0s\\\hline
    \end{tabular}
    \caption{Do HXH with all-sim-reduce TA.}
    % \label{tab:h4}
\end{table}

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|}\hline
       n & G & sB & sA & tB & tA & time & x\\\hline
       13 & 21 & 27 & 413 & 33 & 273 & 0.1s & 0.0s\\\hline
       15 & 24 & 31 & 802 & 38 & 532 & 0.4s & 0.0s\\\hline
       17 & 27 & 35 & 1575 & 43 & 1047 & 1.7s & 0.0s\\\hline
       19 & 30 & 39 & 3116 & 48 & 2074 & 7.9s & 0.0s\\\hline
       21 & 33 & 43 & 6193 & 53 & 4125 & 32s & 0.0s\\\hline
       23 & 36 & 47 & 12342 & 58 & 8224 & 2m45s & 0.0s\\\hline
    \end{tabular}
    \caption{Do MOBV with CTA.}
    \label{tab:h5}
\end{table}

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|}\hline
       n & G & sB & sA & tB & tA & time & x\\\hline
       13 & 21 & 27 & 204 & 33 & 267 & 0.1s & 0.0s\\\hline
       15 & 24 & 31 & 398 & 38 & 525 & 0.3s & 0.0s\\\hline
       17 & 27 & 35 & 784 & 43 & 1039 & 0.7s & 0.0s\\\hline
       19 & 30 & 39 & 1554 & 48 & 2065 & 1.6s & 0.0s\\\hline
       21 & 33 & 43 & 3092 & 53 & 4115 & 4.1s & 0.0s\\\hline
       23 & 36 & 47 & 6166 & 58 & 8213 & 13s & 0.0s\\\hline
       25 & 39 & 51 & 12312 & 63 & 16407 & 56s & 0.0s\\\hline
    \end{tabular}
    \caption{Do MOBV with TA.}
    \label{tab:h6}
\end{table}

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|}\hline
       n & G & sB & sA & tB & tA & time & x\\\hline
       13 & 21 & 27 & 413 & 33 & 273 & 0.1s & 0.0s\\\hline
       15 & 24 & 31 & 802 & 38 & 532 & 0.4s & 0.0s\\\hline
       17 & 27 & 35 & 1575 & 43 & 1047 & 2.1s & 0.0s\\\hline
       19 & 30 & 39 & 3116 & 48 & 2074 & 10s & 0.0s\\\hline
       21 & 33 & 43 & 6193 & 53 & 4125 & 38s & 0.0s\\\hline
       23 & 36 & 47 & 12342 & 58 & 8224 & 2m57s & 0.0s\\\hline       
    \end{tabular}
    \caption{Do MOBV with all-sim-reduce CTA.}
    % \label{tab:h4}
\end{table}

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|}\hline
       n & G & sB & sA & tB & tA & time & x\\\hline
       13 & 21 & 27 & 403 & 33 & 267 & 0.4s & 0.0s\\\hline
       15 & 24 & 31 & 790 & 38 & 525 & 2.1s & 0.0s\\\hline
       17 & 27 & 35 & 1561 & 43 & 1039 & 8.5s & 0.0s\\\hline
       19 & 30 & 39 & 3100 & 48 & 2065 & 38s & 0.0s\\\hline
       21 & 33 & 43 & 6175 & 53 & 4115 & 3m12s & 0.0s\\\hline
    \end{tabular}
    \caption{Do MOBV with all-sim-reduce TA.}
    % \label{tab:h4}
\end{table}

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|}\hline
       n & G & sB & sA & tB & tA & time & x\\\hline
       100 & 100 & 201 & 501 & 301 & 893 & 5.2s & 0.0s\\\hline
       200 & 200 & 401 & 1001 & 601 & 1793 & 44s & 0.0s\\\hline
       300 & 300 & 601 & 1501 & 901 & 2693 & 2m28s & 0.0s\\\hline
       400 & 400 & 801 & 2001 & 1201 & 3593 & 6m10s & 0.0s\\\hline
    \end{tabular}
    \caption{Do GHZall with all-sim-reduce CTA.}
    % \label{tab:h4}
\end{table}

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|}\hline
       n & G & sB & sA & tB & tA & time & x\\\hline
       7 & 7 & 15 & 269 & 22 & 388 & 0.0s & 0.0s\\\hline
       8 & 8 & 17 & 526 & 25 & 773 & 0.3s & 0.0s\\\hline
       9 & 9 & 19 & 1039 & 28 & 1542 & 2.2s & 0.0s\\\hline
       10 & 10 & 21 & 2064 & 31 & 3079 & 22s & 0.0s\\\hline
       11 & 11 & 23 & 4113 & 34 & 6152 & 6m11s & 0.0s\\\hline
    \end{tabular}
    \caption{Do GHZall with all-sim-reduce TA.}
    % \label{tab:h4}
\end{table}

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|}\hline
       n & G & sB & sA & tB & tA & time & x\\\hline
       7 & 7 & 15 & 198 & 22 & 388 & 0.0s & 0.0s\\\hline
8 & 8 & 17 & 391 & 25 & 773 & 0.0s & 0.0s\\\hline
9 & 9 & 19 & 776 & 28 & 1542 & 0.0s & 0.0s\\\hline
10 & 10 & 21 & 1545 & 31 & 3079 & 0.0s & 0.0s\\\hline
11 & 11 & 23 & 3082 & 34 & 6152 & 0.1s & 0.0s\\\hline
12 & 12 & 25 & 6155 & 37 & 12297 & 0.2s & 0.0s\\\hline
13 & 13 & 27 & 12300 & 40 & 24586 & 0.4s & 0.0s\\\hline
14 & 14 & 29 & 24589 & 43 & 49163 & 1.1s & 0.0s\\\hline
15 & 15 & 31 & 49166 & 46 & 98316 & 2.4s & 0.0s\\\hline
16 & 16 & 33 & 98319 & 49 & 196621 & 6.6s & 0.0s\\\hline
17 & 17 & 35 & 196624 & 52 & 393230 & 13s & 0.0s\\\hline
18 & 18 & 37 & 393233 & 55 & 786447 & 34s & 0.0s\\\hline
19 & 19 & 39 & 786450 & 58 & 1572880 & 1m11s & 0.0s\\\hline
    \end{tabular}
    \caption{Do GHZall with CTA.}
    % \label{tab:h4}
\end{table}

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|}\hline
       n & G & sB & sA & tB & tA & time & x\\\hline
       7 & 7 & 15 & 261 & 22 & 388 & 0.0s & 0.0s\\\hline
       8 & 8 & 17 & 518 & 25 & 773 & 0.1s & 0.0s\\\hline
       9 & 9 & 19 & 1031 & 28 & 1542 & 0.6s & 0.0s\\\hline
       10 & 10 & 21 & 2056 & 31 & 3079 & 3.2s & 0.0s\\\hline
       11 & 11 & 23 & 4105 & 34 & 6152 & 15s & 0.0s\\\hline
       12 & 12 & 25 & 8202 & 37 & 12297 & 1m0s & 0.0s\\\hline
       13 & 13 & 27 & 16395 & 40 & 24586 & 3m35s & 0.0s\\\hline
    \end{tabular}
    \caption{Do GHZall with TA.}
    % \label{tab:h4}
\end{table}

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|}\hline
       n & G & sB & sA & tB & tA & time & x\\\hline
       100 & 100 & 201 & 302 & 201 & 299 & 1.7s & 0.0s\\\hline
       200 & 200 & 401 & 602 & 401 & 599 & 15s & 0.0s\\\hline
       300 & 300 & 601 & 902 & 601 & 899 & 56s & 0.0s\\\hline
       400 & 400 & 801 & 1202 & 801 & 1199 & 2m15s & 0.0s\\\hline
    \end{tabular}
    \caption{Do GHZzero with all-sim-reduce CTA.}
    % \label{tab:h4}
\end{table}

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|}\hline
       n & G & sB & sA & tB & tA & time & x\\\hline
       100 & 100 & 201 & 302 & 201 & 299 & 1.0s & 0.0s\\\hline
       200 & 200 & 401 & 602 & 401 & 599 & 8.6s & 0.0s\\\hline
       300 & 300 & 601 & 902 & 601 & 899 & 28s & 0.0s\\\hline
       400 & 400 & 801 & 1202 & 801 & 1199 & 1m17s & 0.0s\\\hline
       500 & 500 & 1001 & 1502 & 1001 & 1499 & 2m28s & 0.0s\\\hline
    \end{tabular}
    \caption{Do GHZzero with all-sim-reduce TA.}
    % \label{tab:h4}
\end{table}

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|}\hline
       n & G & sB & sA & tB & tA & time & x\\\hline
       100 & 100 & 201 & 299 & 201 & 299 & 2.0s & 0.0s\\\hline
       200 & 200 & 401 & 599 & 401 & 599 & 15s & 0.0s\\\hline
       300 & 300 & 601 & 899 & 601 & 899 & 55s & 0.0s\\\hline
       400 & 400 & 801 & 1199 & 801 & 1199 & 2m11s & 0.0s\\\hline
    \end{tabular}
    \caption{Do GHZzero with CTA.}
    % \label{tab:h4}
\end{table}

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|}\hline
       n & G & sB & sA & tB & tA & time & x\\\hline
       100 & 100 & 201 & 299 & 201 & 299 & 1.3s & 0.0s\\\hline
       200 & 200 & 401 & 599 & 401 & 599 & 10s & 0.0s\\\hline
       300 & 300 & 601 & 899 & 601 & 899 & 36s & 0.0s\\\hline
       400 & 400 & 801 & 1199 & 801 & 1199 & 1m32s & 0.0s\\\hline
       500 & 500 & 1001 & 1499 & 1001 & 1499 & 3m5s & 0.0s\\\hline
    \end{tabular}
    \caption{Do GHZzero with TA.}
    % \label{tab:h4}
\end{table}

==> parameterized_with_hamiltonian.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-0.0mm}
\section{Towards Parameterized Verification of Quantum Circuits}\label{sec:paramterizedquantum}
\vspace{-0.0mm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Let us now move to verification of \emph{parameterized circuits}, i.e., checking
correctness of a~(typically) infinite family of quantum circuits with
a~similar structure (differing in the number of qubits).
To the best of our knowledge, parameterized verification of quantum circuits has
not been addressed by any fully automated approach so far.
%\ol{is this true?}\yfc{yes, unless you know something that we overlooked}
In this section, we will show that the use of \lstas enables automated
verification of a~certain class of parameterized circuits.
% One potential use of \lsta is parameterized verification of quantum circuits, that
% is, to check the correctness of a~whole infinite family of quantum circuits with
% a~similar structure (differing in the number of qubits).
In particular, 
we first demonstrate how to use \lstas to verify the parameterized GHZ
circuit~\cite{GreenbergerHZ89} and proceed to the verification of
other circuits used in practice, such as circuits implementing parameterized diagonal
Hamiltonian simulation or fermionic unitary evolution.
At the end, we will discuss the challenges and a direction towards a~complete framework
for parameterized circuit verification.

%*******************************************************************************
\vspace{-0.0mm}
\subsection{Verification of the Parameterized GHZ Circuit}\label{sec:GHZ}
\vspace{-0.0mm}
%*******************************************************************************

An $n$-qubit \emph{GHZ state} (for $n \geq 1$) is a~state of the form
$\frac{\ket{0^n}+\ket{1^n}}{\sqrt{2}}$ and an~\lsta recognizing such states can be
found in~\cref{fig:H0n}. 
% are states from the set $\{\frac{\ket{0^n}+\ket{1^n}}{\sqrt{2}}\mid
% n \geq 1\}$ and a CTA recognizing such states can be found
% \ol{does it allow all states (n=1, n=2 , ... )?} \ja{yes in this case}
An $n$-qubit \emph{GHZ circuit} is shown in \cref{fig:GHZcircuit}; it first
executes the $H_1$ gate and then the sequence of gates $\cnot^{1}_{2}$,
$\cnot^{2}_{3},\ldots, \cnot^{n-1}_{n}$.
The number of $\cnot$ gates involved is $n-1$. 
The circuit transforms a~quantum state of the form $\ket{0^n}$ (represented by the \lsta in
\cref{fig:0n}) to $\frac{\ket{0^n}+\ket{1^n}}{\sqrt{2}}$ (represented
by the \lsta in \cref{fig:H0n}).
To execute this family of circuits, we need to support parameterized quantum gates, which
is generally hard but still feasible in our framework for some cases.
In particular, we introduce the \emph{parameterized $\cnotof n$ gate}, which
implements the sequence of $n-1$ $ \cnot$ gates on~$n$ qubits
(cf.~\cref{fig:GHZcircuit,fig:paramCNOT}).
We will now describe how the effect of such a~parameterized gate is computed on
an~\lsta representing a~set of quantum states.

\figGHZ %%%%%%%%%%%%%%%%%%%%%%%%%%

\fbox{$\cnot(n)$ gate} In~\cref{alg:StaircasesCNOT}, we introduce a~procedure to
build an \lsta $\cnotof{n}(\aut)$
representing the set of states after executing the $\cnotof n$ gate on all
qubits\footnote{One can generalize the algorithm to be applied only on a
continuous subset of qubits in a~straightforward manner, and also
extend it to a~more complex, yet regular, pattern.}.
% $\cnot^{1}_{2}$, $\cnot^{2}_{3},\ldots \cnot^{n-1}_{n}$. 
Recall that the effect of applying the $\cnot^{i}_{i+1}$ gate on a state has the same effect of applying an $X^{i+1}$ gate on the $1$-subtree below every node labeled $x_i$.
Moreover, performing $X$ gate to all qubits of a state, i.e., the $X^{\otimes
n}$ gate, reverses the corresponding vector of amplitudes, e.g., from
$(a,b,c,d)^T$ to $(d,c,b,a)^T$ or, equivalently, reverses all amplitude values of the tree.
Thus, in~\cref{alg:StaircasesCNOT}, we first construct a~primed
version~$\overline \aut = X^{\otimes n}(\aut)$, which encodes trees obtained by reversing the amplitude values of states in $\lang(\aut)$. 
Such an~\lsta~$\overline \aut$ can be constructed from $\aut$ by swapping the two bottom
states of all non-leaf transitions (Lines~\ref{ln:cxn:reverse_start}--\ref{ln:cxn:reverse_end}). 
The resulting automaton is then obtained by combining~$\aut$ and~$\overline \aut$ such
that the right-hand bottom state of $\aut$ is reconnected to the corresponding state
of $\overline \aut$ (Line~\ref{ln:cxn:reconnect_one}), i.e., jumping to
$\overline \aut$ when the
control qubit has value~$1$, and the left-hand bottom state of $\overline \aut$ is reconnected
to the corresponding state of $\aut$ (Line~\ref{ln:cxn:reconnect_two}), i.e.,
jumping back to the original \lsta when control qubit has value~$0$.


%the left-hand side children of nodes are matched using transitions from~$\aut$ and the right-hand side children are matched using transitions from~$\overline \aut$.
% Then the transitions are constructed as keeping the left children in the original automation and switching the right children to the bar version.

%\ol{lemma about correctness?}
{\small
 \begin{restatable}{theorem}{stairCNOTs}\label{thm:stairCNOTs} 
$\lang( \cnot(n)(\aut) )  = \{\cnot^{n-1}_n(\cdots \cnot^1_2 (T)\cdots ) \mid  T\in \lang(\aut) \}
$
and $|\cnot(n)(\aut)|=2|\aut|$.
 \end{restatable}
}

\fbox{Other parameterized gates}  Our framework supports not only $\cnot(n)$,
but also $X^{\otimes n}$, $(D^{1, \omega^m_N})^{\otimes n}$, $\cnot(n)^{-1}$,
and alternating patterns of $\cnot$ gates. We will introduce $\cnot(n)^{-1}$
below. For more details, interested readers can refer to our supplementary
materials. 


\fbox{Non-parameterized gates}  To implement standard (non-parameterized) gates (applied on qubits at a~fixed
offset from the beginning or end, e.g.~$n-3$), one can just use the algorithms
from \cref{sec:quantum_states_and_gates} preceded by an \emph{unfolding
operation} and followed by \emph{folding}. 

\paragraph{Folding and unfolding of \lsta.} Our construction of
\lsta quantum gate operations targeting qubit $x_t$ requires explicitly assigned
index numbers to the first $t$ qubits. We can obtain the explicit qubit
numbering by \emph{unfolding} the transitions for $t$ layers from the root
states and labeling them in order from $x_1$ to $x_t$. One way to do this is to
create $t$ copies of the \lsta $\aut$ and name them $\aut_1$ to $\aut_t$.
Next, we rename the transition symbols of $\aut_i$ from $x$ to $x_i$ and states
from $s$ to $s_i$ for $1 \leq i \leq t$. After that, we connect these \lstas and form an unfolded one.
Starting from $\aut_1$, for each state $s_1$ that can be reached from root
states in one step, we replace it with $s_2$ and thus jump to $\aut_2$. We then
find a~one-step reachable state from $s_2$ and jump to $s_3$, and repeat this
process until we jump from $\aut_t$ to $\aut$. We can unfold the last qubit
$x_t$  using a similar construction. 
The \lsta can be \emph{folded} again by replacing all indexed qubit symbols
$x_i$ with $x$ and (optionally) running a~reduction algorithm. 

To verify the parameterized GHZ circuit, we begin by using the precondition $P$ provided in the \lsta of \cref{fig:0n}. Next, we apply the $\hadam_1$ operation using \cref{algo:u_gate_single} and reduce the output. We then run \cref{alg:StaircasesCNOT} on this \lsta to obtain $\post{C}(P)$. Finally, we check for inclusion against the postcondition $Q$ in \cref{fig:H0n}.

%
% \ol{incorporate this somewhere? say it is done by a procedure similar to the one of sec. 4 and an analogous bottom-up procedure?~~~~~~~~~~~    }
% Let $\aut = \tuple{Q,\Sigma,\Delta,\rootstates,\ell}$ be a~CTA representing an
% infinite set of quantum states parameterized by the number of qubits~$n \geq 1$. 
% Since $n \geq 1$, we may without loss of generality assume that
% %
% \begin{inparaenum}
%   \item initial states only appear (in a run) as roots, i.e., $\not\exists
%     \delta \in \Delta $ such that $\mathtt{bottom}(\delta) \cap \rootstates
%     \neq \emptyset$; and
%   \item there is no leaf transition from the initial states, i.e.,
%     $\not\exists \delta \in \Delta_0$ such that $\mathtt{top}(\delta) \in
%     \rootstates$. 
% \end{inparaenum}
% %
% Then $\Delta$ can be decomposed as $\Delta = \Delta_{i=1} \cup \Delta_{i>1} \cup \Delta_0$, where $\Delta_{i=1}=\{ \delta \in \Delta_{\neq 0} \mid \mathtt{top}(\delta) \in \rootstates \}$ and $\Delta_{i>1} = \Delta_{\neq 0} \setminus \Delta_{i=1}$. 
% Thus, one can apply any $1$-qubit gate on the first qubit of the states recognized by the CTA directly via the algorithms constructed in~\cref{sec:quantum_states_and_gates} without unfolding the CTA.

%%%%%%%%%%%%%%%%%%%%%%%
% Staircases CNOT
%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\algStaircasesCNOT}[0]{
\begin{algorithm}[t]
\caption{Application of the $\cnotof n$ gate on an \lsta}
\label{alg:StaircasesCNOT} 
\KwIn{An \lsta $\aut = \tuple{Q,\Sigma,\Delta,\rootstates}$ representing a parameterized set of quantum states}
\KwOut{An \lsta $\cnotof{n}(\aut)$}
Build $\overline \aut= \tuple{\overline Q,\Sigma, \overline \Delta, \overline
  \rootstates}$, a barred copy of~$\aut$ with
\label{ln:cxn:reverse_start}\\
  \hspace*{2mm}$\overline \Delta = \{ \ctranstreenoset{\overline q} {f}
  {\overline{q_r},\overline{q_l}}{C} \mid \ctranstreenoset {q} {f} {q_l,q_r}{C} \in \Delta \} \cup
  \{ \ctranstreenoset {\overline q}{c}{}{C} \mid \ctranstreenoset {q}{c}{}{C} \in
  \Delta$\tcp*[r]{$\overline \aut = \pauliX^{\otimes n} (\aut)$}
\label{ln:cxn:reverse_end}

% Build $\aut'= X^{\otimes n} (\aut)= \tuple{Q',\Sigma, \Delta', \rootstates'}$, where $\overline\Delta= \{ \ctranstreenoset{\overline{q}} {f} {\overline{q_r},\overline{q_l}}{C} \mid \ctranstreenoset {q} {f} {q_l,q_r}{C} \in \Delta \} \cup \{ \ctranstreenoset {\overline{q}}{c}{}{C} \mid \ctranstreenoset {q}{c}{}{C} \in \Delta \}$\;

% $\overline{(\bullet)}: Q \cup \overline{Q} \to Q \cup \overline{Q}$ be an involution, i.e., $\overline{\overline{q}} =q, \; \forall q$\;
%$\overline{\Delta}_{\neq 0} := \{ \ctranstreenoset{\overline{q}} {f} {\overline{q_r},\overline{q_l}}{C} \mid \ctranstreenoset {q} {f} {q_l,q_r}{C} \in \Delta_{\neq 0} \}$\;
%$\overline{\Delta}_0:= \{ \ctranstreenoset {\overline{q}}{c}{}{C} \mid \ctranstreenoset {q}{c}{}{C} \in \Delta_0 \}$\;
$\Delta^R := \{ \ctranstreenoset {q}{f}{q_l,\overline{q_r}}{C} \mid \ctranstreenoset
  {q}{f}{q_l,q_r}{C} \in \Delta \}\cup {}$\label{ln:cxn:reconnect_one}\\
\hspace*{9mm}$\{ \ctranstreenoset{ \overline q }{f}{q_r,\overline{q_l} }{C} \mid
  \ctranstreenoset{\overline q}{f}{\overline{q_r},\overline{q_l} }{C} \in
  \overline \Delta \} \cup \Delta_0 \cup \overline{\Delta_0}$\label{ln:cxn:reconnect_two}\;
\ol{what is $\Delta_0$?}\;
% \begin{align*}
% \Delta^R &:= \{ \delta^R=\ctranstree {q}{f}{q_l,\overline{q_r}}{C} \mid \delta=\ctranstree {q}{f}{q_l,q_r}{C} \in \Delta_{\neq 0} \} \\
%     &\cup \{ \delta^R= \ctranstree{ \overline{q} }{f}{\overline{\overline{q}_l },\overline{q}_r }{C} \mid \delta = \ctranstree{\overline{q}}{f}{\overline{q}_l,\overline{q}_r }{C} \in \overline{\Delta}_{\neq 0} \} \cup \Delta_0 \cup \overline{\Delta}_0
% \end{align*}
\Return{$\aut^R = \tuple{Q \uplus \overline Q,\Sigma,\Delta^R,\rootstates}$}\;
\end{algorithm}
}
%%%%%%%%%%%%%%%%%%%%
\algStaircasesCNOT
%%%%%%%%%%%%%%%%%%%%%



\hide{
Formally, $\mathrm{CNOT}(n)(\aut) := \aut^R =\tuple{Q^R,\Sigma,\Delta^R,\rootstates,\ell^R} $, where we let 
\begin{enumerate}
    \item $\overline{Q}:= \{ \overline{q} \mid q\in Q \}$
    \item $\overline{(\bullet)}: Q \cup \overline{Q} \to Q \cup \overline{Q}$ be an involution, i.e., $\overline{\overline{q}} =q, \; \forall q$.
    \item $\overline{\Delta}_{\neq 0} := \{ \overline{\delta}= \ctranstree {\overline{q}} {f} {\overline{q_r},\overline{q_l}}{C} \mid \delta = \ctranstree {q} {f} {q_l,q_r}{C} \in \Delta_{\neq 0} \}$.
    \item $\overline{\Delta}_0:= \{ \overline{\delta}= \ctranstree {\overline{q}}{c}{}{C} \mid \delta=\ctranstree {q}{c}{}{C} \in \Delta_0 \}$
\end{enumerate}
Set $Q^R := Q \cup \overline{Q}$ and 
\begin{align*}
    \Delta^R &:= \{ \delta^R=\ctranstree {q}{f}{q_l,\overline{q_r}}{C} \mid \delta=\ctranstree {q}{f}{q_l,q_r}{C} \in \Delta_{\neq 0} \} \\
    &\cup \{ \delta^R= \ctranstree{ \overline{q} }{f}{\overline{\overline{q}_l },\overline{q}_r }{C} \mid \delta = \ctranstree{\overline{q}}{f}{\overline{q}_l,\overline{q}_r }{C} \in \overline{\Delta}_{\neq 0} \} \cup \Delta_0 \cup \overline{\Delta}_0
\end{align*}
\yfc{explain this procedure}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\figHamiltonianSimulation}[0]{
\begin{figure}[t]%{0.58\textwidth}
% \begin{subfigure}[b]{0.45\textwidth}
% \centering
% \scalebox{0.55}{\parbox{.3\linewidth}{
% \begin{align*}
%     \ctranstree {q}{x}{0_r,r_1}{C_r} 
%     &&\ctranstree {q}{x}{l,0_l}{C_l}
%     &&\ctranstree {r_1}{x}{\hat{0}_r,\hat{r}_2}{\hat{C}_r}
%     &&\ctranstree {\hat{r}_2}{1}{}{C}\\
%     \ctranstree {r_1}{x}{0_r,r_2}{C_r}
%     &&\ctranstree {r_2}{x}{l,0_l}{C_l} 
%     &&\ctranstree {r_2}{x}{\hat{l},\hat{0}_l}{\hat{C}_l}
%     &&\ctranstree {\hat{l}}{1}{}{C}\\
%     \ctranstree {r_2}{x}{0_r,r_1}{C_r}
%     &&\ctranstree {0_r}{x}{0_l,0_l}{C_l} 
%     &&\ctranstree {l}{x}{\hat{l},\hat{0}_l}{\hat{C}_l} 
%     &&\ctranstree {\hat{0}_l}{0}{}{C}\\
%     \ctranstree {0_r}{x}{0_r,0_r}{C_r}
%     &&\ctranstree {l}{x}{l,0_l}{C_l}
%     &&\ctranstree {0_r}{x}{\hat{0}_r,\hat{0}_r}{\hat{C}_r}
%     &&\ctranstree {\hat{0}_r}{0}{}{C}\\
%     \ctranstree {l}{x}{0_r,r_1}{C_r}  
%     &&\ctranstree {0_l}{x}{0_l,0_l}{C_l}
%     &&\ctranstree {0_l}{x}{\hat{0}_l,\hat{0}_l}{\hat{C}_l} &&\\
%     \ctranstree {0_l}{x}{0_r,0_r}{C_r} 
%     &&
%     &&
%     &&
% \end{align*}
% }}
% \caption{The CTA $\aut_{even}$ of basis states $\ket{x}$ with even $1$'s}    
% \label{fig:evenparityautomata}
% \end{subfigure}
% \hfill
% \begin{subfigure}[b]{0.45\textwidth}
% \centering
% \scalebox{0.5}{
% \begin{quantikz}
%   \lstick{$\ket{x_1}$} &\gate{\mathrm{Ph}(-at)} &\ctrl{1}   & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \ctrl{1} & \qw\\
%   \lstick{$\ket{x_2}$} &\qw      &\targ{}     & \ctrl{1} & \qw & \qw & \qw & \qw & \qw & \ctrl{1} &\targ{} & \qw \\
%   \lstick{$\ket{x_3}$}  & \qw  &\qw   &\targ{}     & \qw & \qw & \qw & \qw & \qw & \targ{} & \qw & \qw \\  
%   \ldots\\
%   \lstick{$\ket{x_{n-2}}$} &\qw & \qw & \qw   & \ctrl{1} & \qw & \qw & \qw & \ctrl{1} & \qw & \qw & \qw \\
%   \lstick{$\ket{x_{n-1}}$} &\qw & \qw & \qw   & \targ{} & \ctrl{1} & \qw & \ctrl{1} & \targ{} & \qw & \qw & \qw \\
%   \lstick{$\ket{x_n}$} &\qw & \qw & \qw   & \qw & \targ{} & \gate{\mathrm{R}_Z(2bt) } & \targ{} & \qw & \qw & \qw & \qw \\ 
%   \end{quantikz}
% }
%   \caption{A~circuit implementing the unitary operator $U(t)=e^{-i t (a\identity^{\otimes n} + b\pauliZ^{\otimes n} ) }$}
%   \label{fig:HamiltonianZ}
% \end{subfigure}
\begin{subfigure}[b]{0.34\textwidth}
\centering
 \scalebox{0.75}{
 \begin{quantikz}[row sep=0.3cm]
   \lstick{$\ket{x_1}$}     & \qw      & \qw      & \qw      & \qw      & \ctrl{1} & \qw\\
   \lstick{$\ket{x_2}$}     & \qw      & \qw      & \qw      & \ctrl{1} & \targ{}  & \qw\\
   \lstick{$\ket{x_3}$}     & \qw      & \qw      & \qw & \targ{}  & \qw      & \qw\\
  \cdots \\
   \lstick{$\ket{x_{n-2}}$} & \qw      & \ctrl{1} & \qw  & \qw      & \qw      & \qw \\
   \lstick{$\ket{x_{n-1}}$} & \ctrl{1} & \targ{}  & \qw      & \qw      & \qw      & \qw\\
   \lstick{$\ket{x_n}$}     & \targ{}  & \qw      & \qw      & \qw      & \qw      & \qw\\
  \end{quantikz}}
\vspace{-3mm}
\caption{The $\cnotof{n}^{-1}$ gate.} \label{fig:cnotinv}
\end{subfigure}
\begin{subfigure}[b]{0.65\textwidth}
\centering
\scalebox{0.75}{
\begin{quantikz}
  \lstick{$\ket{x_1}$} &\gate{\mathrm{Ph}(-at)} &\gate[3]{\cnotof n}   & \qw & \gate[3]{\cnotof{n}^{-1}} & \qw \\
  \lstick{$\ket{x_2}$}\lstick[label style={xshift=-1mm,yshift=-8mm}]{\vdots} & \qw & \qw & \lstick[label style={xshift=1mm,yshift=-8mm}]{\vdots}\qw & \qw & \qw\lstick[label style={xshift=1mm,yshift=-8mm}]{\vdots}\\[10mm]
  \lstick{$\ket{x_n}$} & \qw  &\qw   &\gate{\gateRZ(2bt) }     & \qw & \qw\\  
  \end{quantikz}
}
\vspace{-3mm}
  \caption{A~circuit implementing the unitary operator $U(t)=e^{-i t
  (a\identity^{\otimes n} + b\pauliZ^{\otimes n} ) }$. In the experimental
  evaluation, we use $a = b = -\frac{\pi} 2$ and $t=1$.}
  \label{fig:HamiltonianZ}
\end{subfigure}
\vspace{-6mm}
\caption{A~circuit for diagonal Hamiltonian simulation.}
% \caption{Verifying diagonal Hamiltonian simulation circuit}
\label{fig:HamiltonianSimulation}
\end{figure}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Reverse Staircases CNOT
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\algReverseStaircasesCNOT}[0]{
\begin{algorithm}
\caption{Application of the $\cnotof{n}^{-1}$ gate on an \lsta}
\label{alg:ReversedStaircasesCNOT}
\KwIn{An \lsta $\aut = \tuple{Q,\Sigma,\Delta,\rootstates}$ representing a parameterized set of quantum states}
\KwOut{An \lsta $\cnotof{n}^{-1}(\aut)$}
Build $\overline \aut= \tuple{\overline Q,\Sigma,
  \overline\Delta, \overline\rootstates}$ with\\
  \hspace*{2mm}$\overline\Delta= \{ \ctranstreenoset{\overline{q}} {f} {\overline{q_r},\overline{q_l}}{C} \mid \ctranstreenoset {q} {f} {q_l,q_r}{C} \in \Delta \} \cup \{ \ctranstreenoset {\overline{q}}{c}{}{C} \mid \ctranstreenoset {q}{c}{}{C} \in \Delta \}$\tcp*[r]{$\overline \aut = \pauliX^{\otimes n} (\aut)$}

$\Delta^R := \{ \ctranstreenoset {q}{f}{q_l,\overline{q_r}}{C} \mid \ctranstreenoset {q}{f}{q_l,q_r}{C} \in \Delta \}\cup {}$\\
\hspace*{9mm}$\{ \ctranstreenoset{ \overline{q} }{f}{\overline{q_r},q_l }{C}
  \mid \ctranstreenoset{\overline{q}}{f}{\overline{q_r},\overline{q_l} }{C} \in
  \overline{\Delta} \} \cup \Delta_0 \cup
  \overline{\Delta}_0$\label{ln:cxn_rev:two}\;
% $\Delta^R := \{\ctranstree{q}{f}{q_l,\overline{q_r}}{C} \mid \ctranstree{q}{f}{q_l,q_r}{C} \in \Delta_{\neq 0} \cup \overline{\Delta}_{\neq 0} \} \cup \Delta_0 \cup \overline{\Delta}_0$\;
\Return{$\aut^R = \tuple{Q \uplus \overline{Q},\Sigma,\Delta^R,\rootstates}$}\;
\end{algorithm}
}



%*******************************************************************************
\vspace{-0.0mm}
\subsection{Verification of Diagonal Hamiltonian Simulation Circuit}\label{sect:Hamiltonian}
\vspace{-0.0mm}
%*******************************************************************************

In many areas, like \emph{quantum chemistry} or \emph{material science}, it is
often important to figure out how a~quantum system will evolve from some given
initial state, for instance, a~basis state~\cite{McArdleEA20,Moll18,CaoRO19,ValahuOMNRMPYBHTK23}. 
In these areas, the modeled systems can often be described using the so-called
\emph{Hamiltonians}, i.e., $2^n \times 2^n$ \emph{Hermitian} matrices (a~matrix
is Hermitian if it is equal to its conjugate transpose)~\cite{McArdleEA20}.
Any Hamiltonian can be decomposed into a linear combination of tensor
products of identity and Pauli gates ($\identity$, $\pauliX$, $\pauliY$,
$\pauliZ$)~\cite[Chapter~4.7]{NielsenC16}.
% \ol{citation needed; is it true?} \ja{because they form a basis of the vector
% space of $2^n \times 2^n$ Hermitian matrices, can be found in any quantum
% computing textbook, maybe c.f. Nelsen and Chuang section 4.7 or de wolf}
Hamiltonians are, in general, not unitary matrices, so they cannot be directly
used as a~part of a~quantum circuit.
The evolution of a~system described by a~Hamiltonian~$\Ham$ in time~$t$ can,
however, be computed
% , be efficiently simulated \ol{what does that mean?} \ja{use quantum computer to simulate (compute interesting values like energy of) the system described by the Hamiltonian}
by a~quantum
circuit implementing the unitary operator $U(t) = e^{-it\Ham}$; this approach is
called \emph{Hamiltonian simulation}~\cite{NielsenC16}.

\figHamiltonianSimulation   %%%%%%%%%%%%%%%%%%%%%

\algReverseStaircasesCNOT 
Our framework allows to express \emph{parameterized Hamiltonian simulation} of
certain \emph{diagonal} Hamiltonians.
A~Hamiltonian~$\Ham$ is diagonal if~$\Ham$ is a~diagonal matrix.
% (non-zero entries can only be on the diagonal).
The class of Hamiltonians that we support are those that can be described as a~linear
combination of the $n$-fold identity
and Pauli~$\pauliZ$ gates, i.e., $\Ham = a \identity^{\otimes n} + b\pauliZ^{\otimes n}$
for $a,b \in \reals$ and~$n \in \nat$ being the parameter.
% \ol{can it be more general?}
% \ja{for diagonal $H$ there might be also summands like $ A_1\otimes A_2 \otimes \cdots \otimes A_n, A_i \in \{\identity ,\pauliZ \}$ }
Such a~Hamiltonian can be simulated by the unitary operator $U(t) = e^{-it\Ham}$ represented by the circuit in
\cref{fig:HamiltonianZ} (see \cref{app:diagonal_hamiltonian} for the formal
derivation of correctness of the circuit \ol{supplementary materials?}). %\ol{check the appendix is OK}
We verify the correctness of this circuit against the precondition $\{\ket{0^n}\mid n \geq 1\}$ (\cref{fig:0n}), the usual initial states of quantum computers.

\fbox{$\cnotof{n}^{-1}$ gate} Application of the $\cnotof{n}^{-1}$ gate on an
\lsta is in \cref{alg:ReversedStaircasesCNOT}.
In the circuit, we use the $\cnotof{n}^{-1}$ gate, the inverse of
$\cnotof{n}$, which corresponds to the circuit in \cref{fig:cnotinv}.
To execute such a circuit, we also need to provide an
implementation of the parameterized $\cnotof{n}^{-1}$ gate.
The procedure is similar to the one in \cref{alg:StaircasesCNOT}. The only
difference is that on Line~\ref{ln:cxn_rev:two}, the right-hand bottom state of $\overline \aut$ is
reconnected to the corresponding state of $\aut$, not the left-hand side state,
i.e., we jump back to the original \lsta when the value of the control qubit is~$1$.



{
\small
 \begin{restatable}{theorem}{stairCNOTsinv}\label{thm:stairCNOTsinv} 
 $
 \lang( \cnot(n)^{-1}(\aut) )  = \{\cnot^{1}_2(\cdots \cnot^{n-1}_n (T)\cdots ) \mid  T\in \lang(\aut) \}
 $
 and $|\cnot(n)^{-1}(\aut)| = 2|\aut|$.
 \end{restatable}
}


%\ol{lemma about correctness?}

% \ol{example with the EVEN CTA?}

%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\figFermionicA}[0]{
\begin{figure}[thb]
\resizebox{\linewidth}{!}{
\input{figs/1fermionic.tikz}
}
\caption{A standard circuit performing a single fermionic excitation.}
\label{fig:1fermionic}
\end{figure}
}

\newcommand{\figFermionicB}[0]{
\begin{figure}[t]
\resizebox{\linewidth}{!}{
\input{figs/2fermionic.tikz}
}
\caption{Part of the circuit performing a double fermionic excitation.
  See~\cite[Fig.~11]{YordanovADB20} for the whole circuit.}
\label{fig:2fermionic}
\end{figure}
}
%*******************************************************************************
\vspace{-0.0mm}
\subsection{Verification of Fermionic Unitary Evolutions}\label{sec:fermionic}
\vspace{-0.0mm}
%*******************************************************************************

\figFermionicA

Two major challenges in the practical realization of the \emph{variational
quantum eigensolver} on \emph{noisy intermediate-scale quantum} (NISQ)
computers are the design of \emph{ansatz} states (i.e., states that serve as
the initial \emph{guess} of the final value) and the construction of efficient
circuits to prepare these states for a~parameterized number of qubits.
Most ansatz states considered by the quantum chemistry and material science
communities correspond to applying a series of \emph{fermionic unitary
evolutions} to an initial reference state~\cite{YordanovADB20}.
These evolutions are referred as single and double \emph{fermionic
excitations} and can be transformed via \emph{Jordan-Wigner} encoding into the
quantum circuits in \cref{fig:1fermionic} and \cref{fig:2fermionic}~\cite{YordanovADB20}.
Both of these circuits can be executed using the algorithms introduced
previously (for the double fermionic excitation, we need to unfold the first
and the last two qubits of the \lsta representing the 
set of states). We verify the correctness of this circuit against the precondition $\{\ket{0^n}\mid n \geq 1\}$ (\cref{fig:0n}).
%
% For the double one, since one needs at least $4$ qubits, we may fix transitions in CTA corresponding to the first and last two qubits. Then one can construct algorithms for applying any single qubit gate on them as in the previous section. Thus, the double fermionic excitation circuit can be executed too. 

\figFermionicB

%\subsection{Summary and outlook of the parameterized verification}
% Apart from applying any $1$-qubit unitary on the first and last qubits and staircases $\mathrm{CNOT}$ operators in both directions, we have also constructed several other operations interpreting the quantum circuits, c.f.~\cref{app:parameterizedverification}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\tablePar}[0]{
\begin{wraptable}[8]{r}{4.4cm}
\caption{Results for verification of parameterized circuits}
\vspace{-3mm}
\label{table:exp_par}
% \resizebox*{\dimexpr\textwidth-4\baselineskip\relax}{!}{
% \scalebox{0.6}{
\resizebox{\linewidth}{!}{
\input{table_par.tex}
}
\end{wraptable}
}

%*******************************************************************************
\vspace{-0.0mm}
\subsection{Evaluation and Discussion}
\vspace{-0.0mm}
%*******************************************************************************

\tablePar    %%%%%%%%%%%%%%%

We extended \tool to support parameterized verification and used it to verify
the circuits from \cref{fig:paramCNOT}, \cref{fig:HamiltonianZ},
\cref{fig:1fermionic}, and \cref{fig:2fermionic}.
The results are given in~\cref{table:exp_par}.
All of these families of circuits could be verified efficiently.
Even though the sets of encoded quantum states are infinitely large, their symbolic
representation is compact (less than 10 states and 20 transitions). 

Our current approach only supports a limited set of parameterized quantum gates.
Particularly, the gate $H^{\otimes n}$ is currently beyond our capability
because applying it to the states $\{\ket{0^n}\}$ would create an infinite set
of constant symbols $\{\frac{1}{\sqrt{2}^{k}} \mid k\in \nat\}$. To address this
issue, one idea is to introduce a variable $b$ to represent the current basis
state\footnote{Similar idea is already used in the
path-sum approach~\cite{amy2018towards,Chareton2021}. \ol{approach for what?}} and use it in the leaf symbol.
For the aforementioned example, it would be enough to use the singleton set $\{\frac{1}{\sqrt{2}^{{|b|}}}\}$ as the leaf symbols, where $|b|$ is equivalent to the number of used qubits. We are planning to explore this direction further in the future.

\ol{we should have some more exciting conclusion of the section on param. verif.}







==> table_all_old.tex <==
\begin{tabular}{crrrrrrrrrrrrrrrrrrrrrrr}\hline
\toprule
  &&&& \multicolumn{8}{c}{\usecase{Verification}} & \multicolumn{6}{c}{\usecase{Missing gate bug}} & \multicolumn{6}{c}{\usecase{Flipped gate bug}}\\
  \cmidrule(lr){5-12} \cmidrule(lr){13-18} \cmidrule(lr){19-24}
  &&&& \multicolumn{3}{c}{\tool} & \multirow{2}{*}{\autoq} & \multirow{2}{*}{\sliqsim} & \multirow{2}{*}{SV-Sim} & \multirow{2}{*}{\symqv} & \multirow{2}{*}{\caal} & \multicolumn{3}{c}{\tool} & \multirow{2}{*}{\autoq}& \multirow{2}{*}{\symqv} & \multirow{2}{*}{\caal}& \multicolumn{3}{c}{\tool} & \multirow{2}{*}{\autoq} & \multirow{2}{*}{\symqv} & \multirow{2}{*}{\caal}\\
  \cmidrule(lr){5-7} \cmidrule(lr){13-15} \cmidrule(lr){19-21}
  & \multicolumn{1}{c}{$n$} & \multicolumn{1}{c}{\textbf{\#q}} & \multicolumn{1}{c}{\textbf{\#G}} & \multicolumn{1}{c}{$\post{C}$} & \multicolumn{1}{c}{$\subseteq$}  & \multicolumn{1}{c}{total} &&&&&& \multicolumn{1}{c}{$\post{C}$} & \multicolumn{1}{c}{$\subseteq$}  & \multicolumn{1}{c}{total}&&&& \multicolumn{1}{c}{$\post{C}$} & \multicolumn{1}{c}{$\subseteq$}  & \multicolumn{1}{c}{total}\\
\midrule
  \multirow{ 5}{*}{\rotatebox[origin=c]{90}{\bvsingbench}}
 & 95 & 96 & 241 & 0.2s & 0.0s & \textbf{0.2s} & 4.3s &\bestresult 0.0s & \error & \timeout & \timeout& 0.2s                           & 0.0s                                & \bestresult \textbf{0.2s}      & 4.8s                     & \timeout & \timeout & 0.2s & 0.0s & \bestresult \textbf{0.2s} & 4.4s & \timeout & \timeout\\
 & 96 & 97 & 243 & 0.2s & 0.0s & \textbf{0.2s} & 4.6s &\bestresult 0.0s & \error & \timeout & \timeout& 0.2s                           & 0.0s                                & \bestresult \textbf{0.2s}      & 4.8s                     & \timeout & \timeout & 0.2s & 0.0s & \bestresult \textbf{0.2s} & 4.6s & \timeout & \timeout\\
 & 97 & 98 & 246 & 0.3s & 0.0s & \textbf{0.3s} & 4.7s &\bestresult 0.0s & \error & \timeout & \timeout& 0.2s                           & 0.0s                                & \bestresult \textbf{0.2s}      & 5s                       & \timeout & \timeout & 0.3s & 0.0s & \bestresult \textbf{0.3s} & 4.7s & \timeout & \timeout\\
 & 98 & 99 & 248 & 0.2s & 0.0s & \textbf{0.2s} & 4.9s &\bestresult 0.0s & \error & \timeout & \timeout& 0.3s                           & 0.0s                                & \bestresult \textbf{0.3s}      & 5.1s                     & \timeout & \timeout & 0.3s & 0.0s & \bestresult \textbf{0.3s} & 4.8s & \timeout & \timeout\\
 & 99 & 100 & 251 & 0.3s & 0.0s & \textbf{0.3s} & 5s &\bestresult 0.0s & \error & \timeout & \timeout & 0.2s                           & 0.0s                                & \bestresult \textbf{0.2s}      & 5.2s                     & \timeout & \timeout & 0.2s & 0.0s & \bestresult \textbf{0.2s} & 5s   & \timeout & \timeout\\
\midrule
  \multirow{ 5}{*}{\rotatebox[origin=c]{90}{\bvmultbench}}
 & 9  & 19 & 30 & 0.0s & 0.0s & \bestresult \textbf{0.0s} & 2.8s  & \timeout & 53s      & \timeout & \timeout & 0.0s                           & 0.0s                                & \bestresult \textbf{0.0s}      & 2.9s                     & \timeout & \timeout\\
 & 10 & 21 & 33 & 0.0s & 0.0s & \bestresult \textbf{0.0s} & 8s    & \timeout & \timeout & \timeout & \timeout & 0.0s                           & 0.0s                                & \bestresult \textbf{0.0s}      & 7.3s                     & \timeout & \timeout\\
 & 11 & 23 & 36 & 0.0s & 0.0s & \bestresult \textbf{0.0s} & 23s   & \timeout & \timeout & \timeout & \timeout & 0.0s                           & 0.0s                                & \bestresult \textbf{0.0s}      & 44s                      & \timeout & \timeout\\
 & 12 & 25 & 39 & 0.0s & 0.0s & \bestresult \textbf{0.0s} & 1m11s & \timeout & \timeout & \timeout & \timeout & 0.0s                           & 0.0s                                & \bestresult \textbf{0.0s}      & 1m58s                    & \timeout & \timeout\\
 & 13 & 27 & 42 & 0.0s & 0.0s & \bestresult \textbf{0.0s} & 4m45s & \timeout & \timeout & \timeout & \timeout & 0.0s                           & 0.0s                                & \bestresult \textbf{0.0s}      & \timeout                 & \timeout & \timeout\\
\midrule
\multirow{ 5}{*}{\rotatebox[origin=c]{90}{\ghzsingbench}}
 & 64  & 64  & 64  & 0.0s & 0.0s & \bestresult \textbf{0.0s} & 0.3s  & \bestresult 0.0s & \error & \timeout & \timeout & 0.0s                           & 0.0s                                & \bestresult \textbf{0.0s}      & 0.4s                     & \timeout & \timeout & 0.0s & 0.0s &\bestresult \textbf{0.0s} & 0.3s & \timeout & \timeout\\
 & 128 & 128 & 128 & 0.1s & 0.0s & \textbf{0.1s}             & 2.5s  & \bestresult 0.0s & \error & \timeout & \timeout & 0.1s                           & 0.0s                                & \bestresult \textbf{0.1s}      & 2.5s                     & \timeout & \timeout & 0.1s & 0.0s &\bestresult \textbf{0.1s} & 2.7s & \timeout & \timeout\\ 
 & 256 & 256 & 256 & 0.8s & 0.0s & \textbf{0.8s}             & 20s   & \bestresult 0.0s & \error & \timeout & \timeout & 0.8s                           & 0.0s                                & \bestresult \textbf{0.8s}      & 20s                      & \timeout & \timeout & 0.7s & 0.0s &\bestresult \textbf{0.7s} & 20s & \timeout & \timeout\\  
 & 384 & 384 & 384 & 1.9s & 0.0s & \textbf{1.9s}             & 1m10s & \bestresult 0.1s & \error & \timeout & \timeout & 1.9s                           & 0.0s                                & \bestresult \textbf{1.9s}      & 1m12s                    & \timeout & \timeout & 1.7s & 0.0s &\bestresult \textbf{1.7s} & 1m9s & \timeout & \timeout\\ 
 & 512 & 512 & 512 & 3.6s & 0.0s & \textbf{3.6s}             & 2m49s & \bestresult 0.1s & \error & \timeout & \timeout & 3.6s                           & 0.0s                                & \bestresult \textbf{3.6s}      & 2m59s                    & \timeout & \timeout & 3.3s & 0.0s &\bestresult \textbf{3.3s} & 2m52s & \timeout & \timeout\\
\midrule
  \multirow{ 5}{*}{\rotatebox[origin=c]{90}{\ghzmultbench}}
 & 8   & 8   & 8   & 0.0s & 0.0s & \bestresult \textbf{0.0s} & 0.1s     & 1.5s     & \bestresult 0.0s & \timeout & \timeout & 0.0s                           & 0.0s                                & \bestresult \textbf{0.0s}      & 0.2s                     & \timeout & 30s      & 0.0s & 0.0s & \bestresult \textbf{0.0s} & 0.1s     & \timeout & 32s\\     
 & 16  & 16  & 16  & 0.0s & 0.0s & \bestresult \textbf{0.0s} & \timeout & \timeout & 1m37s            & \timeout & \timeout & 0.0s                           & 0.0s                                & \bestresult \textbf{0.0s}      & \timeout                 & \timeout & \timeout & 0.0s & 0.0s & \bestresult \textbf{0.0s} & \timeout & \timeout & 55s\\     
 & 32  & 32  & 32  & 0.0s & 0.0s & \bestresult \textbf{0.0s} & \timeout & \timeout & \error           & \timeout & \timeout & 0.0s                           & 0.0s                                & \bestresult \textbf{0.0s}      & \timeout                 & \timeout & 1m28s    & 0.0s & 0.0s & \bestresult \textbf{0.0s} & \timeout & \timeout & 1m27s\\   
 & 64  & 64  & 64  & 0.1s & 0.0s & \bestresult \textbf{0.1s} & \timeout & \timeout & \error           & \timeout & \timeout & 0.1s                           & 0.0s                                & \bestresult \textbf{0.1s}      & \timeout                 & \timeout & \timeout & 0.1s & 0.0s & \bestresult \textbf{0.1s} & \timeout & \timeout & 3m7s\\    
 & 128 & 128 & 128 & 0.6s & 0.0s & \bestresult \textbf{0.6s} & \timeout & \timeout & \error           & \timeout & \timeout & 0.5s                           & 0.0s                                & \bestresult \textbf{0.5s}      & \timeout                 & \timeout & \timeout & 0.6s & 0.0s & \bestresult \textbf{0.6s} & \timeout & \timeout & \timeout\\
\midrule
  \multirow{ 5}{*}{\rotatebox[origin=c]{90}{\groversingbench}}
 & 12 & 24 & 5215   & 1.3s & 0.0s & \bestresult \textbf{1.3s} & 10s      & \timeout & \timeout & \timeout & \timeout & 1.3s                           & 0.0s                                & \bestresult \textbf{1.3s}      & 10s                      & \timeout & \missing  & 1.5s  & 0.0s & \bestresult \textbf{1.5s}  & 11s      & \timeout & \missing \\
 & 14 & 28 & 12217  & 3.8s & 0.0s & \bestresult \textbf{3.8s} & 32s      & \timeout & \timeout & \timeout & \timeout & 3.9s                           & 0.0s                                & \bestresult \textbf{3.9s}      & 32s                      & \timeout & \missing  & 4.1s  & 0.0s & \bestresult \textbf{4.1s}  & 35s      & \timeout & \missing \\
 & 16 & 32 & 28159  & 10s  & 0.0s & \bestresult \textbf{10s}  & 1m28s    & \timeout & \error   & \timeout & \timeout & 16s                            & 0.0s                                & \bestresult \textbf{16s}       & 2m35s                    & \timeout & \missing  & 11s   & 0.0s & \bestresult \textbf{11s}   & 1m41s    & \timeout & \missing \\
 & 18 & 36 & 63537  & 26s  & 0.0s & \bestresult \textbf{26s}  & 4m3s     & \timeout & \error   & \timeout & \timeout & 45s                            & 0.0s                                & \bestresult \textbf{45s}       & \timeout                 & \timeout & \missing  & 28s   & 0.0s & \bestresult \textbf{28s}   & 4m36s    & \timeout & \missing \\
 & 20 & 40 & 141527 & 1m8s & 0.0s & \bestresult \textbf{1m8s} & \timeout & \timeout & \error   & \timeout & \timeout & 1m28s                          & 0.0s                                & \bestresult \textbf{1m28s}     & \timeout                 & \timeout & \missing  & 1m13s & 0.0s & \bestresult \textbf{1m13s} & \timeout & \timeout & \missing \\
\midrule
  \multirow{ 5}{*}{\rotatebox[origin=c]{90}{\grovermultbench}}
 & 6  & 18 & 357  & 0.2s & 0.0s & \bestresult \textbf{0.2s}  & 3.1s     & \timeout & 38s      & \timeout & \timeout & 0.2s                           & 0.0s                                & \bestresult \textbf{0.2s}      & 3.6s                     & \timeout & \timeout & 0.5s  & 0.0s & \bestresult \textbf{0.5s}  & 10s      & \timeout & \timeout\\
 & 7  & 21 & 552  & 0.8s & 0.0s & \bestresult \textbf{0.8s}  & 10s      & \timeout & \timeout & \timeout & \timeout & 0.9s                           & 0.0s                                & \bestresult \textbf{0.9s}      & 12s                      & \timeout & \missing & 1.8s  & 0.0s & \bestresult \textbf{1.8s}  & 31s      & \timeout & \missing\\       
 & 8  & 24 & 939  & 3.0s & 0.1s & \bestresult \textbf{3.1s}  & 38.1s    & \timeout & \timeout & \timeout & \timeout & 3.0s                           & 0.1s                                & \bestresult \textbf{3.1s}      & 44s                      & \timeout & \missing & 7.1s  & 0.2s & \bestresult \textbf{7.3s}  & \timeout & \timeout & \missing\\       
 & 9  & 27 & 1492 & 9.7s & 0.8s & \bestresult \textbf{10.5s} & 2m20s    & \timeout & \timeout & \timeout & \timeout & 9.8s                           & 0.7s                                & \bestresult \textbf{10.5s}     & 3m38s                    & \timeout & \missing & 25s   & 1.1s & \bestresult \textbf{26.1s} & \timeout & \timeout & \missing\\       
 & 10 & 30 & 2433 & 36s  & 3.3s & \bestresult \textbf{39.3s} & \timeout & \timeout & \error   & \timeout & \timeout & 36s                            & 3.2s                                & \bestresult \textbf{39.2s}     & \timeout                 & \timeout & \missing & 1m28s & 4.2s & \bestresult \textbf{1m32s} & \timeout & \timeout & \missing\\       
\midrule
  \multirow{ 5}{*}{\rotatebox[origin=c]{90}{\hhbench}}
 & 12  & 12  & 24  & 0.0s & 0.0s & \bestresult \textbf{0.0s} & 40s      & 1m51s    & 0.5s   & \timeout & \timeout & 0.0s                           & 0.0s                                & \bestresult \textbf{0.0s}      & 39s                      & \timeout & \timeout\\
 & 13  & 13  & 26  & 0.0s & 0.0s & \bestresult \textbf{0.0s} & 2m35s    & \timeout & 2.1s   & \timeout & \timeout & 0.0s                           & 0.0s                                & \bestresult \textbf{0.0s}      & 2m15s                    & \timeout & \error\\
 & 64  & 64  & 128 & 0.2s & 0.0s & \bestresult \textbf{0.2s} & \timeout & \timeout & \error & \timeout & \timeout & 0.2s                           & 0.0s                                & \bestresult \textbf{0.2s}      & \timeout                 & \timeout & \timeout\\
 & 128 & 128 & 256 & 0.9s & 0.0s & \bestresult \textbf{0.9s} & \timeout & \timeout & \error & \timeout & \timeout & 1.0s                           & 0.0s                                & \bestresult \textbf{1s}        & \timeout                 & \timeout & \timeout\\
 & 256 & 256 & 512 & 4.4s & 0.0s & \bestresult \textbf{4.4s} & \timeout & \timeout & \error & \timeout & \timeout & 4.9s                           & 0.0s                                & \bestresult \textbf{4.9s}      & \timeout                 & \timeout & \timeout\\
\midrule
  \multirow{ 5}{*}{\rotatebox[origin=c]{90}{\hxhbench}}
 & 10 & 10 & 30  & 0.0s & 0.0s & \bestresult \textbf{0.0s} & 1.8s     & 11s      & \bestresult 0.0s & \timeout & \timeout & 0.0s                           & 0.0s                                & \bestresult \textbf{0.0s}      & 1.1s                     & \timeout & \timeout\\
 & 11 & 11 & 33  & 0.0s & 0.0s & \bestresult \textbf{0.0s} & 4.3s     & 34s      & 0.2s             & \timeout & \timeout & 0.0s                           & 0.0s                                & \bestresult \textbf{0.0s}      & 5.3s                     & \timeout & \timeout\\
 & 12 & 12 & 36  & 0.0s & 0.0s & \bestresult \textbf{0.0s} & 11.1s    & 1m51s    & 0.7s             & \timeout & \timeout & 0.0s                           & 0.0s                                & \bestresult \textbf{0.0s}      & 15s                      & \timeout & \timeout\\
 & 13 & 13 & 39  & 0.0s & 0.0s & \bestresult \textbf{0.0s} & 36.3s    & \timeout & 2.9s             & \timeout & \timeout & 0.0s                           & 0.0s                                & \bestresult \textbf{0.0s}      & 1m51s                    & \timeout & \timeout\\
 & 99 & 99 & 297 & 0.7s & 0.0s & \bestresult \textbf{0.7s} & \timeout & \timeout & \error           & \timeout & \timeout & 0.7s                           & 0.0s                                & \bestresult \textbf{0.7s}      & \timeout                 & \timeout & \timeout\\
\midrule
  \multirow{ 5}{*}{\rotatebox[origin=c]{90}{\mctoffolibench}}
 %& 8 & 16 & 15 & 0.0s/0.0s & 0.0s/0.0s & \textbf{0.0s/0.0s} & 0.0s & \timeout & 7.7s & \timeout & \timeout\\
 %& 10 & 20 & 19 & 0.0s/0.0s & 0.0s/0.0s & \textbf{0.0s/0.0s} & 0.0s & \timeout & \timeout & \timeout & \timeout\\
 %& 12 & 24 & 23 & 0.0s/0.0s & 0.0s/0.0s & \textbf{0.0s/0.0s} & 0.0s & \timeout & \timeout & \timeout & \timeout\\
 %& 14 & 28 & 27 & 0.0s/0.0s & 0.0s/0.0s & \textbf{0.0s/0.0s} & 0.1s & \timeout & \timeout & \timeout & \timeout\\
 %& 16 & 32 & 31 & 0.0s/0.0s & 0.0s/0.0s & \textbf{0.0s/0.0s} & 0.2s & \timeout & \error & \timeout & \timeout\\
 & 8  & 16 & 15 & 0s/0s & 0s/0s & \bestresult \textbf{0.0s/0.0s} & \bestresult 0.0s/0.0s & \timeout & 7.7s     & \timeout & \timeout & 0s/0s                          & 0s/0s                               & \bestresult \textbf{0.0s/0.0s} & \bestresult 0.0s/0.0s    & \timeout & \timeout & 0s/0s & 0s/0s &\bestresult \textbf{0.0s/0.0s} &\bestresult 0.0s & \timeout & \timeout\\
 & 10 & 20 & 19 & 0s/0s & 0s/0s & \bestresult \textbf{0.0s/0.0s} & \bestresult 0.0s/0.0s & \timeout & \timeout & \timeout & \timeout & 0s/0s                          & 0s/0s                               & \bestresult \textbf{0.0s/0.0s} & \bestresult 0.0s/0.0s    & \timeout & \timeout & 0s/0s & 0s/0s &\bestresult \textbf{0.0s/0.0s} &\bestresult 0.0s & \timeout & \timeout\\
 & 12 & 24 & 23 & 0s/0s & 0s/0s & \bestresult \textbf{0.0s/0.0s} & \bestresult 0.0s/0.0s & \timeout & \timeout & \timeout & \timeout & 0s/0s                          & 0s/0s                               & \bestresult \textbf{0.0s/0.0s} & \bestresult 0.0s/0.0s    & \timeout & \timeout & 0s/0s & 0s/0s &\bestresult \textbf{0.0s/0.0s} &\bestresult 0.0s & \timeout & \timeout\\
 & 14 & 28 & 27 & 0s/0s & 0s/0s & \bestresult \textbf{0.0s/0.0s} & 0.1s/0.1s             & \timeout & \timeout & \timeout & \timeout & 0s/0s                          & 0s/0s                               & \bestresult \textbf{0.0s/0.0s} & 0.1s/0.1s                & \timeout & \timeout & 0s/0s & 0s/0s &\bestresult \textbf{0.0s/0.0s} & 0.1s & \timeout & \timeout\\           
 & 16 & 32 & 31 & 0s/0s & 0s/0s & \bestresult \textbf{0.0s/0.0s} & 0.1s/0.2s             & \timeout & \error   & \timeout & \timeout & 0s/0s                          & 0s/0s                               & \bestresult \textbf{0.0s/0.0s} & 0.1s/0.1s                & \timeout & \timeout & 0s/0s & 0s/0s &\bestresult \textbf{0.0s/0.0s} & 0.2s & \timeout & \timeout\\           
\midrule
  \multirow{ 5}{*}{\rotatebox[origin=c]{90}{\oegroverbench}}
 & 2   & 3   & 13  & 0.0s & 0.0s & \bestresult \textbf{0.0s}  & 0.3s     & \missing & \missing & \missing & \missing & 0.0s                           & 0.1s                                & \bestresult \textbf{0.1s}      & \timeout                 & 12s      & 46s\\
 & 18  & 36  & 157 & 0.0s & 0.0s & \bestresult \textbf{0.0s}  & 2.0s     & \missing & \missing & \missing & \missing & 0.0s                           & 0.0s                                & \bestresult \textbf{0.0s}      & 2.3s                     & \timeout & \timeout\\
 & 50  & 100 & 445 & 2.2s & 0.0s & \bestresult \textbf{2.2s}  & 49s      & \missing & \missing & \missing & \missing & 2.4s                           & 0.1s                                & \bestresult \textbf{2.5s}      & 55s                      & \timeout & \timeout\\
 & 75  & 150 & 671 & 7.4s & 0.1s & \bestresult \textbf{7.5s}  & 3m35s    & \missing & \missing & \missing & \missing & 7.7s                           & 0.1s                                & \bestresult \textbf{7.8s}      & \timeout                 & \timeout & \timeout\\
 & 100 & 200 & 895 & 17s  & 0.1s & \bestresult \textbf{17.1s} & \timeout & \missing & \missing & \missing & \missing & 18s                            & 0.1s                                & \bestresult \textbf{18.1s}     & \timeout                 & \timeout & \timeout\\
\bottomrule
\end{tabular}


==> temp.tex <==
\subsection*{Specifying Properties using CTA}
Below, we give a few examples to demonstrate how to use CTA for specifying properties. The first example is the verification of the Bernstein–Vazirani algorithm that learns a secret string encoded in a function. Our circuit consists of $2n$ qubits. The first $n$ qubits are for generating the function that encodes the secret string and the next $n$ qubits are the work tape for the Bernstein–Vazirani algorithm. 
The precondition should encodes the set of states $\{\ket{s0^n}\mid s\in \mathbb{B}^n\}$ and the postcondition should be the states $\{\ket{ss}\mid s\in \mathbb{B}^n\}$. Both can be expressed using CTA. Notice that the qubit order would affect the size of CTA encoding. Here we alternate the $2n$ qubits and use the order $q_1q_{1+n}\ldots q_{n}q_{2n}$ to obtain a CTA of $XX$ states for the encoding of post-condition. \yfc{It might be too early to talk about qubit ordering here.}

In another example, we verify the correctness of a circuit implementing multi-control Toffoli gates, which converts a state $\ket{x_1\ldots x_{n-1}x_n}$ to the state $\ket{x_1\ldots x_{n-1}(x_1 \oplus x_2\oplus\ldots \oplus x_n)}$. We can check the correctness using the pre-condition $\{\ket{s_1\ldots s_{n-1}0}\mid s_1,\ldots, s_{n-1}\in \mathbb{B}\}$ and post-condition $\{\ket{s_1\ldots s_{n-1}b}\mid s_1,\ldots, s_{n-1}\in \mathbb{B} \wedge b= s_1\oplus\ldots\oplus s_{n-1}\}$. Notice that this pair of pre- and post-conditions is insufficient to guarantee the functional correctness of this circuit, but is useful for diagnosing this implementation.


Target: CTA's expressiveness 
\begin{itemize}
    \item All BV
    \item MCToffolli?
    \item Grover > 90\% (say this is hard using pathsum)
    \item Grover iteration increase
    \item Equivalence
\end{itemize}
% \hide{To illustrate this, we provide an example of how to encode the infinite set of GHZ quantum states $\{\frac{1}{\sqrt{2}}(\ket{0^n}+\ket{1^n})\mid n>0\}$, which is a representation of the \emph{maximally entangled state} named after Greenberger, Horne, and Zeilinger. This is achieved using the CTA as shown in figure \ref{fig:fbtree2}.}

We further demonstrate how to use CTAs for
% In \cref{sec:paramterizedquantum}, we demonstrate the usefulness of CTA in
parameterized verification of quantum circuits and provide three non-trivial
examples. We have extended the approach to support various types of
parameterized quantum gates, including applying $\cnot$ gates to every
consecutive qubit in either a~top-down or bottom-up manner. With these
additional gates, we could prove the correctness of GHZ circuits~\cite{GreenbergerHZ89} for any number
of qubits using CTAs. We also tested the approach on a~more complex circuit that
performs the \emph{diagonal Hamiltonian simulation}~\cite{Stuart21}, and some
circuits performing
\emph{fermionic unitary evolution}~\cite{YordanovADB20}, which is frequently used in quantum chemistry.
Our experimental results demonstrate that our algorithm is indeed efficient: we
have solved problems with sizes orders of magnitude larger than what the
state-of-the-art tool \autoq~\cite{ChenCLLTY23,ChenCLLT23} can handle and also
successfully verified several parameterized quantum circuits.



\newcommand{\decisiontreecontrolled}[0]{
\begin{wrapfigure}[7]{r}{0.65\textwidth}\label{fig:decision_tree2}
  \vspace{-4mm}
\begin{minipage}{\linewidth}
\begin{subfigure}[b]{0.32\linewidth}
\centering
    \begin{tikzpicture}[anchor=base]
    \node {$x_1$}[sibling distance = 1cm, level distance = 0.8cm]
        child  {node {$x_2$} edge from parent [dashed, sibling distance = .7cm]
            child  {node {$a$} edge from parent [dashed]}
            child {node {$b$} edge from parent [solid]};
            }
        child {node {$x_2$} edge from parent [solid, sibling distance = .7cm]
            child  {node {$c$} edge from parent [dashed]}
            child {node {$d$}}};
    \end{tikzpicture}
    \vspace{-2mm}
    \caption{The state $q$.}
\end{subfigure}
\begin{subfigure}[b]{0.32\linewidth}
\centering
    \begin{tikzpicture}[anchor=base]
    \node {$x_1$}[sibling distance = 1cm, level distance = 0.8cm]
        child  {node {$x_2$} edge from parent [dashed, sibling distance = .7cm]
            child  {node {$a$} edge from parent [dashed]}
            child {node {$b$} edge from parent [solid]};
            }
        child {node {$x_2$} edge from parent [solid, sibling distance = .7cm]
            child  {node {$d$} edge from parent [dashed]}
            child {node {$c$}}};
    \end{tikzpicture}
    \vspace{-2mm}
    \caption{Applied $\cnot^1_2$.}
    \label{fig:CX1_decision_tree}
\end{subfigure}
\begin{subfigure}[b]{0.32\linewidth}
\centering
    \begin{tikzpicture}[anchor=base]
    \node {$x_1$}[sibling distance = 1cm, level distance = 0.8cm]
        child  {node {$x_2$} edge from parent [dashed, sibling distance = .7cm]
            child  {node {$a$} edge from parent [dashed]}
            child {node {$d$} edge from parent [solid]};
            }
        child {node {$x_2$} edge from parent [solid, sibling distance = .7cm]
            child  {node {$c$} edge from parent [dashed]}
            child {node {$b$}}};
    \end{tikzpicture}
    \vspace{-2mm}
    \caption{Applied $\cnot^2_1$.}
    \label{fig:CX2_decision_tree}
\end{subfigure}
\end{minipage}
    \vspace{-4mm}
\caption{The effect of applying controlled quantum gates to the state $q$.}
\end{wrapfigure}
}

\newcommand{\decisiontreesinglegate}[0]{
\begin{wrapfigure}[9]{r}{0.7\textwidth}%\label{fig:decision_tree}
\vspace{-5mm}
\begin{minipage}{\linewidth}
\begin{subfigure}[b]{0.24\linewidth}
\centering
    \begin{tikzpicture}[anchor=base]
    \node {$x_1$}[sibling distance = 1cm, level distance = 0.8cm]
        child  {node {$x_2$} edge from parent [dashed, sibling distance = .7cm]
            child  {node {$a$} edge from parent [dashed]}
            child {node {$b$} edge from parent [solid]};
            }
        child {node {$x_2$} edge from parent [solid, sibling distance = .7cm]
            child  {node {$c$} edge from parent [dashed]}
            child {node {$d$}}};
    \end{tikzpicture}
    \caption{The state $q$.}
    \label{fig:decision_tree}
\end{subfigure}
\begin{subfigure}[b]{0.24\linewidth}
\centering
    \begin{tikzpicture}[anchor=base]
    \node {$x_1$}[sibling distance = 1cm, level distance = 0.8cm]
        child  {node {$x_2$} edge from parent [dashed, sibling distance = .7cm]
            child  {node {$b$} edge from parent [dashed]}
            child {node {$a$} edge from parent [solid]};
            }
        child {node {$x_2$} edge from parent [solid, sibling distance = .7cm]
            child  {node {$d$} edge from parent [dashed]}
            child {node {$c$}}};
    \end{tikzpicture}
    \caption{Applied $\pauliX_2$.}
    \label{fig:X_decision_tree}
\end{subfigure}
\begin{subfigure}[b]{0.24\linewidth}
\centering
    \begin{tikzpicture}[anchor=base]
    \node {$x_1$}[sibling distance = 1cm, level distance = 0.8cm]
        child  {node {$x_2$} edge from parent [dashed, sibling distance = .5cm]
            child  {node {$a$} edge from parent [dashed]}
            child {node {$-b$} edge from parent [solid]};
            }
        child {node {$x_2$} edge from parent [solid, sibling distance = .5cm]
            child  {node {$c$} edge from parent [dashed]}
            child {node {$-d$}}};
    \end{tikzpicture}
    \caption{Applied $\pauliZ_2$.}
    \label{fig:Z_decision_tree}
\end{subfigure}
\begin{subfigure}[b]{0.24\linewidth}
\centering
    \begin{tikzpicture}[anchor=base]
    \node {$x_1$}[sibling distance = 1cm, level distance = 0.8cm]
        child  {node {$x_2$} edge from parent [dashed, sibling distance = .5cm]
            child  {node {$\frac{a+c}{\sqrt{2}}$} edge from parent [dashed]}
            child {node {$\frac{b+d}{\sqrt{2}}$} edge from parent [solid]};
            }
        child {node {$x_2$} edge from parent [solid, sibling distance = .5cm]
            child  {node {$\frac{a-c}{\sqrt{2}}$} edge from parent [dashed]}
            child {node {$\frac{b-d}{\sqrt{2}}$}}};
    \end{tikzpicture}
    \caption{Applied $\hadam_1$.}
    \label{fig:H_decision_tree}
\end{subfigure}
\end{minipage}
\vspace{-3mm}
\caption{The effect of applying single-qubit quantum gates to the state $q$. The left-going line means the $0$-branch, and the right-going one is the $1$-branch.}
\end{wrapfigure}
}



%*******************************************************************************
\vspace{-0.0mm}
\subsection{Prior Work on Using Tree Automata for Quantum Circuit Verification}\label{sec:TA}
\vspace{-0.0mm}
%*******************************************************************************

The \autoq framework~\cite{ChenCLLTY23,ChenCLLT23} draws inspiration from symbolic verification and uses tree automata as the symbolic representation of a set of quantum states (decision trees). By utilizing the tree automata inclusion algorithm and the developed gate operations, quantum circuits can be verified fully automatically. Below, we provide the formal definition of tree automata and show their limitation when used in quantum circuit verification, which motivates our current work.

%\paragraph{Trees.} 
%We use a~\emph{ranked alphabet}~$\Sigma$ with arity function $\Arity\colon\Sigma\to\nat$ where $\Sigma$ is a finite set. The \emph{arity} of a symbol $f\in \Sigma$ is $\Arity(f)$. The set of symbols with arity $p$ is denoted by $\Sigma_p$. The set with arity $0$, i.e., $\Sigma_0$, is the set of \emph{constant symbols}. 
%A~\emph{tree} is a~\emph{ground term} over~$\Sigma$.
%For instance, $T = f(f(c_1, c_2), g(f(c_2, c_3), c_1))$ represents
%a~binary tree, with $f,g \in \Sigma_2$ and $c_1,c_2,c_3\in \Sigma_0$.
%The set of \emph{nodes} of a~tree~$T$, denoted as~$\dom(T)$, is defined
%inductively as a~set of words over~$\nat$ such that for every constant
%symbol~$c$, we define $N_c = \{\epsilon\}$, and for every other symbol~$f$ with $n=\Arity(f)-1$, we
%define
%$N_{f(T_0,\ldots,T_n)} = \{\epsilon\} \cup \{a.w \mid a \in \{0,\ldots,n\}  \land w\in
%N_{T_a}\}$, where~$\epsilon$ is the empty word and~`$.$' is concatenation.
%Each tree $T$ is associated with a~labeling function $L_T\colon \nat^* \to \Sigma$, which maps a~node in~$T$ to its label in~$\Sigma$. 
%We call a node $w$ a \emph{leave node} when $L_T(w)\in\Sigma_0$.
%The \emph{height} of a node $w\in \dom(T)$, denoted by $\height(w)$, is the word length of $w$. We say a node $w$ is at tree level $i$ when $\height(w)=i$. We say a tree is \emph{perfect} if all leave nodes have the same height.

%\paragraph{Tree Automata.}
%A~\emph{(nondeterministic finite) tree automaton} (TA) is a~tuple $\aut = \tuple{Q, \Sigma,
%	\Delta, \rootstates}$ where~$Q$ is a~finite set of \emph{states},
%$\Sigma$~is a~ranked alphabet,
%$\rootstates \subseteq Q$ is the set of \emph{root states}, and
%$\Delta=\cup_{i\in\{0,\ldots, n\}}\Delta_i$, for some constant $n\in \nat$, is a set of tree transitions consisting of the set~$\Delta_i$ of $i$-ary \emph{transitions} of the form $\transtree q f
%{q_0,\ldots,q_{i-1}}$,
%for $q, q_0, \ldots q_{i-1} \in Q$. The set~$\Delta_0$ consists of \emph{leaf transitions} of the form $\transtree q {c} {}$ (for a~constant symbol~$c$). We denote by $\Delta_{\neq 0} = \cup_{i\in \{1, \ldots, n\}}\Delta_i$ the set of non-leaf transitions. We call $q$ (resp. $\{q_0,\dots,q_{i-1}\}$) the \emph{top} (resp. \emph{bottom}) of a transition $\delta= \transtree q f
%{q_0,\dots,q_{i-1}}$, and $f$ the \emph{symbol} of $\delta$, denoted as $\mathtt{top}(\delta)$, $\mathtt{bottom}(\delta)$, and $\mathtt{sym}(\delta)$, respectively. We define the \emph{size} of a TA as its number of states, denoted as $|\aut|$.
%We abuse the notation and denote by $\Delta(q)$ the set of transitions whose top state is $q$.

%%------------------------------------------------------------------------------
%\paragraph{Run and Language.}
%A \emph{run} of~$\aut$ on a~tree $T$ is a partial mapping $\run\colon \nat^* \partto \Delta$ such that
%%
%\begin{inparaenum}[(i)]
%  \item  for all leaf nodes $u\in \dom(T)$, we have $\run(u)= \transtree q {L_T(u)} {} \in \Delta_0$, and
%  \item  for all non-leaf nodes $v\in \dom(T)$, we have $\run(v)=\transtree q f
%{q_0,\ldots,q_{\Arity(f)-1}}$ satisfying 
%    \begin{inparaenum}[(1)]
%        \item $f= L_T(v)$ and
%        \item $q_{i} = \mathtt{top}(\run(i.u)) $ for $i \in [0,\Arity(f)-1]$, where $[l,u]$ is the set of integer numbers $\{i\mid l\leq i \leq u\}$.
%          %\ol{undefined notation $[\ldots]$, also $n$ is fixed as sth else}
%    \end{inparaenum}
%\end{inparaenum}
%%
%The run~$\run$ is \emph{accepting} if $\mathtt{top}(\run(\epsilon)) \in \rootstates$ . 
%The \emph{language} $\lang(\aut)$ of~$\aut$ is the set of trees accepted by~$\aut$, i.e.,
%$\langof \aut = \{T \mid \text{there exists an accepting run of } \aut \text{ over } T\}$.

\paragraph{Trees.} 
% \hide{We use $\nat$ to denote the set of natural numbers (including zero) and.
% A ranked alphabet is a set of symbols $\Sigma$ together with a function $\arityof\colon\Sigma\to\nat$ that gives \emph{ranks} to symbols. 
% We let $\Sigma_p = \{f\in\Sigma \mid \arityof f = p\}$ and we call elements of $\Sigma_0$ the \emph{constant symbols} or \emph{leaf symbols}.
% A~\emph{tree} is a finite map $T:\nat^*\rightarrow \Sigma$ that maps \emph{tree nodes} to symbols,
% and satisfies that 
% \begin{inparaenum}
%     \item $\dom(T)$ is prefix closed and
%     \item if $T(v) = f$, then the set $\{vi\in T\mid i\in\nat\}$ of \emph{children} of $v$ equals $\{1,\ldots,\arityof f\}$ ($v$ has no children if $\arityof f = 0$).
% \end{inparaenum}
% Nodes labeled by leaf symbols are called \emph{leaf nodes}.
% The \emph{height} of a node $w\in \dom(T)$, denoted by $\height(w)$, is the word length of $w$. We say a node $w$ is at tree level $i$ when $\height(w)=i$. We say a tree is \emph{perfect} if all leave nodes have the same height.}
In mathematical notation, we use $\nat$ to represent the set of natural numbers
(without~0) and $\natz=\nat\cup\{0\}$.
A ranked alphabet is a set of symbols $\Sigma$ with a corresponding rank given
by a~function $\arity\colon\Sigma\to\natz$. The symbols with the same rank $p$ are grouped together into $\Sigma_p$, and symbols from $\Sigma_0$, with rank zero, are called \emph{constant} or \emph{leaf} symbols. 

A~\emph{tree} is a finite map $T\colon\nat^*\rightarrow \Sigma$ that maps \emph{tree nodes} to symbols in $\Sigma$, and satisfies that
%
\begin{enumerate}
    \item the domain of $T$ is prefix-closed and
    \item if $T(v) = f$ with $\arityof f = n$, then the set of \emph{children} of $v$ equals $\{v.1,\ldots,v.n\}$. \\
(here $.$ denotes the concatenation, and $v$ has no children if $\arityof f = 0$)
\end{enumerate}
Nodes labeled by leaf symbols are called \emph{leaf nodes}. 
A node's \emph{height} is its word length, denoted~$\height(w)$. A node $w$ is at tree level $i$ when $\height(w)=i$. A tree is \emph{perfect} if all leaf nodes have the same height.
We sometimes write trees as terms, e.g., the tree in
\cref{fig:decision_tree} can be written as the term $x_1(x_2(a,b), x_2(c,d))$.

\paragraph{Tree Automata.}
A~\emph{(nondeterministic finite) tree automaton} (TA) is a~tuple $\aut = \tuple{Q, \Sigma,
\Delta, \rootstates}$ where~$Q$ is a~finite set of \emph{states},
$\rootstates \subseteq Q$ is a~set of \emph{root states},
$\Sigma$~is a~ranked alphabet,
$\Delta$ is a~finite set of \emph{tree transitions}
$\delta = \transtree {q} f {q_1,\ldots,q_{n}}$ where $n = \arityof f$ and $q,q_1,\ldots,q_{n}\in Q$. 
We call $q$, $f$, and $\{q_1,\dots,q_{n}\}$ the \emph{top}, the \emph{symbol}, and the \emph{bottom}, respectively, of the transition $\delta$, 
and denote them by $\topof \delta$, $\symof \delta$, and $\botof \delta$, respectively. 
We~denote by $\Delta(q)$ the set of transitions $\delta$ with $\topof \delta = q$.
%
We~denote by $\Delta_i$, for $i\in\natz$, the subset of transitions of $\Delta$ with the symbols of the rank~$i$, we
call elements of $\Delta_0$ \emph{leaf transitions}, and we denote by $\Delta_{\neq 0} = \cup_{i\in \nat}\Delta_i$ the set of \emph{non-leaf transitions}. 
%
We define the \emph{size} of~$\aut$ as its number of states, denoted as $|\aut|$.
%
%
%------------------------------------------------------------------------------
%\paragraph{Run and Language.}
%A \emph{run} of~$\aut$ on a~tree $T$ is a total map $\run\colon \dom(T) \rightarrow Q$ such that for each $v\in \dom(T)$,
%$\transtree {\run(v)} {T(v)} {\run(v.1),\ldots,\run(v.n)} \in \Delta$, where $n = \arityof {T(v)}$. %
%The run is \emph{accepting} if $\rho(\epsilon)\in\rootstates$, the tree $T$ is the accepted by $\aut$, and 
%the \emph{language} of $\aut$ is the set $L(\aut)$ of accepted trees.
%
A \emph{run} of~$\aut$ on a~tree $T$ is a total map $\run\colon \dom(T) \rightarrow \Delta$ such that for each $v\in \dom(T)$, 
$\run(v)$ is of the form $\transtree {q} {T(v)} {\topof{\run(v.1)},\ldots,\topof{\run(v.n)}}$ where $q\in Q$ and $n = \arityof {T(v)}$. %
The run is \emph{accepting} if $\topof{\rho(\epsilon)}\in\rootstates$, the tree $T$ is then \emph{accepted} by $\aut$, and 
the \emph{language} of $\aut$ is the set $\langof \aut$ of trees accepted
by~$\aut$.
We call the class of languages accepted by TAs \emph{regular tree languages}.

%*******************************************************************************
\vspace{-0.0mm}
\subsection{Limitation of TAs}\label{sec:ta_limit}
\vspace{-0.0mm}
%*******************************************************************************

As we mentioned in the introduction, TAs do not allow per-level synchronization
between states. However, for  \emph{compact encoding of quantum states} and
\emph{efficient quantum operations}, which are needed in verification of quantum
circuits, such a~type of synchronization is necessary.

\paragraph{Quantum state encoding.}
Let us consider the set of GHZ states $\{\frac{1}{\sqrt{2}}
(\ket{0^n}+\ket{1^n})\mid n>0\}$, named after Greenberger, Horne, and
Zeilinger~\cite{GreenbergerHZ89}. These quantum states feature maximal
entanglement between qubits. We will explain why it is not possible to represent
them using TAs.
We assume that there is a TA $\aut$ accepting all GHZ states, which is an
infinite set of perfect trees. 
We use~$q^i_l$ and $q^i_r$ to denote the left and right states at level~$1$ of
some accepting run of $\aut$ on a~tree with height~$i$.
Since there are a finite number of states in~$\aut$, and there are infinitely many accepted trees of different heights, there must be two different heights, $i$ and $j$, such that $q^i_l=q^j_l$. 
This leads us to the conclusion that $q^i_l$ has (due to non-determinism) at
least two potential choices of subtrees with different heights below it.
Since there is no synchronizing mechanism between states at the same level,
$q^i_l$ can choose a subtree whose height is different from the height of
$q^i_r$'s subtree. Therefore, $\aut$~can accept a~tree that is not perfect
and, therefore, does not encode a~quantum state.

\ghzstate

\wl{The above example is about parametrization, not about balancing. Another balancing example is that in our benchmarks, the post conditions of (fixed-qubit) GHZall circuits require CTA to be more compact. Maybe give one example to show that the size of CTA << the size of TA. The size of TA should be proven to have a lower bound. Unfortunately, all other circuits can still use only TA to be compact. Reviewer D: To convincingly argue CTA's advantages in parameterized quantum circuit verification, the paper should include a more diverse and quantum-interesting set of examples or stronger arguments for its advantage over other methods beyond AUTOQ.}

\paragraph{Quantum gate operations.}
Per-level synchronization is also necessary for gate operations. Assume we
have a TA~$\aut$ with the transition $\delta\colon \transtree {q} {x_1} {q_0, q_1}$
with $q$ being the only root state, and following $\aut$'s structure, there are
two possible subtrees $x_2(c,d)$ and $x_2(c',d')$ accepted from~$q_1$
(downwards) and only one subtree $x_2(a,b)$ accepted from~$q_0$.
That is, $\aut$~accepts exactly two trees $x_1(x_2(a,b),x_2(c,d))$ and
$x_1(x_2(a,b),x_2(c',d'))$. When we apply $\hadam_1$ (from
\cref{fig:decision_tree} to \cref{fig:H_decision_tree}) to $\aut$, we should
fuse the $0$- and $1$-subtrees under~$x_1$.
$\hadam_1(\aut)$
should then accept exactly two trees:
$x_1(x_2(\frac{a+c}{\sqrt{2}},\frac{b+d}{{\sqrt{2}}}), x_2(\frac{a-c}{\sqrt{2}},\frac{b-d}{{\sqrt{2}}}))$ and $x_1(x_2(\frac{a+c'}{\sqrt{2}},\frac{b+d'}{{\sqrt{2}}}), x_2(\frac{a-c'}{\sqrt{2}},\frac{b-d'}{{\sqrt{2}}}))$.

% <<<<<<< HEAD
A common approach to build $\hadam_1(\aut)$ is to use the ``product construction'' to produce a pair of states that come with annotations on how to merge them.
We might update $\delta$ to $\transtree {q} {x_1} {(q_0, q_1, +), (q_0,q_1,-)}$,
where the product states $(q_0,q_1,\pm)$ mean that we should traverse the trees
under $q_0$ and $q_1$ simultaneously, and $\pm$ denotes how the leaves of the
two trees should be merged. The issue here is that the $q_1$ occurring in $(q_0, q_1, +)$ and $(q_0, q_1, -)$ should always choose the same subtree, either $x_2(c,d)$ or $x_2(c',d')$. Otherwise, it may incorrectly accept the tree
$x_1(x_2(\frac{a+c}{\sqrt{2}},\frac{b+d}{{\sqrt{2}}}), x_2(\frac{a-c'}{\sqrt{2}},\frac{b-d'}{{\sqrt{2}}}))$.
This synchronization cannot be efficiently expressed with TAs, and so the
$\hadam$ gate construction in~\cite{ChenCLLTY23} is exponential, as it
needs to have \mbox{copies of states that ``\emph{remember}'' the synchronization
explicitly.}

\wl{Don't know if we should also put the corresponding picture here or not.}

%They need to handle $x_2(c,d)$ and $x_2(c',d')$ via an explicit encoding.
% \lu{I don't get this... }\yfc{the last sentence or the entire paragraph?}
% =======
% A common approach to build $H_1(\aut)$ is to use the ``product construction'' to produce a pair of states that come with annotations on how to merge them.
% We might update $\delta$ to $\transtree {q} {x_1} {(q_0, q_1, +), (q_0,q_1,-)}$, where the product states $(q_0,q_1,\pm)$ mean that we should traverse the trees under $q_0$ and $q_1$ simultaneously, and $\pm$ denotes how the leaves of the two trees should be merged. The issue here is that the $q_1$ occurs in $(q_0, q_1, +)$ and $(q_0, q_1, -)$ should always choose the same subtree, either $x_2(c,d)$ or $x_2(c',d')$. Otherwise, it may incorrectly accept the tree
% $x_1(x_2(\frac{a+c}{\sqrt{2}},\frac{b+d}{{\sqrt{2}}}), x_1(x_2(\frac{a-c'}{\sqrt{2}},\frac{b-d'}{{\sqrt{2}}}))$.
% This cannot be efficiently expressed using TA, and hence the $\hadam$ gate construction in~\cite{ChenCLLTY23} is exponential. They need to handle $x_2(c,d)$ and $x_2(c',d')$ via an explicit encoding.%\lu{I don't get this... }\yfc{the last sentence or the entire paragraph?}
% >>>>>>> 4e314a9b22cbd8c9d1416431ca06b1c6e611f7ae

\subsection{Quantum parallelism: why quantum can be faster than classical}
The circuit in~\cref{fig:Hcircuit} creates a \emph{uniform superposition} state
(\cref{fig:uniform_superposition}) from the state $\ket{000}$
(\cref{fig:init_state}).
In such a~\emph{uniform superposition} state, each computational basis state has
the same probability of being observed.
Note that a system consisting of $n$ qubits has $2^n$ computational basis states. When a quantum gate is applied to an $n$-qubit state, the gate can update $2^n$ classical states all at once. This is why quantum computing can bring an exponential speed-up, in terms of gate counts, to classical algorithms.

\section{Below is not processed yet}

%
% \begin{equation}\label{def:CTArun}
% | \{\delta\in \Delta(q) \mid \ell(\delta) \subseteq \Col(\transet) \}| = 1\ .
% \end{equation}
%
% That is, $q$ can have only one transition, unambiguously determined, consistent with the colors of $\transet$.

%%%%%%%%%%%%%%%%%%%%%%%%%%
% Example in minipage in order to show figure
%%%%%%%%%%%%%%%%%%%%%%%%%%
% \smallskip
% \noindent
%\begin{minipage}{0.78\textwidth}
\begin{example}[Accepted tree and its run]\label{ex:tree_and_run}
Assume a~TA~$\aut_3$ with~$q$ as its single root state and the following transitions. 
%
\begin{align*}
  \transtree {q} {x_1} {q^1_0, q^1_1} && \transtree {q^1_1} {x_2} {q^2_0, q^2_1} && \transtree {q^2_1} {x_3} {q_0, q_1} && \transtree {q_0} {\algzero} {}\\
  \transtree {q} {x_1} {q^1_1, q^1_0} && \transtree {q^1_1} {x_2} {q^2_1, q^2_0} && \transtree {q^2_1} {x_3} {q_1, q_0} && \transtree {q_1} {\algone} {}\\
  &&\transtree {q^1_0} {x_2} {q^2_0, q^2_0} && \transtree {q^2_0} {x_3} {q_0, q_0}
\end{align*}
%
% \begin{align*}
% \transtree {q} {x_1} {q^1_0, q^1_1}, \transtree {q} {x_1} {q^1_1, q^1_0},\\
% \transtree {q^1_1} {x_2} {q^2_0, q^2_1}, \transtree {q^1_1} {x_2} {q^2_1, q^2_0}, \transtree {q^1_0} {x_2} {q^2_0, q^2_0},\\
% \transtree {q^2_1} {x_3} {q_0, q_1}, \transtree {q^2_1} {x_3} {q_1, q_0}, \transtree {q^2_0} {x_3} {q_0, q_0},\\
% \transtree {q_1} {c_1} {}, \transtree {q_0} {c_0} {}.
% \end{align*}
%
% \input{figs/tree_and_run.tex}

%
\begin{center}
  \input{figs/example_tree.tikz}
  \hspace{15mm}
  \input{figs/example_run.tikz}
\end{center}
Among others, $\aut_3$ accepts the above tree (in the left) with the
run (in the right).
Observe that all tree nodes satisfy the requirement of a valid run. E.g., 
the node $\greenlab{111}$ corresponds to the transition $\transtree {q_0} {\algzero} {}$, $\redlab{01}$ to $\transtree {q^2_0} {x_3} {q_0, q_0}$, and $\bluelab{\epsilon}$ to $\transtree{q} {x_1} {q^1_1, q^1_0}$, etc.

In $\aut_3$, we use states named~$q^n_0$ to denote only subtrees with all
zeros ($\algzero$) in leaves that can be generated from here, and states named~$q^n_1$ to denote only subtrees with a single~$\algone$ in the leaves that can be generated from it.
Intuitively, the TA accepts all trees of the height three with exactly
one~$\algone$ leaf and all other leaves~$\algzero$ (in our encoding of quantum states,
this might correspond to saying that~$\aut_3$ encodes an arbitrary computational basis
state of a~three-qubit system).
\hfill\qed

\end{example}

%That is, the set of transitions taken from the top states in $T$ is unambiguously determined by those top states of transitions from $T$ and by the colors $\Col(T)$. \ja{roots may be confused with roots of $\aut$. we may use top or parent or something else instead?} \yfc{I feel this intuition is a bit miss leading, but I do not know how to fix it atm.}

%
We define the \emph{level} $d$ of a run $\run$ of $\aut$ on a tree $T$ as the set of transitions
$$ \level(\run,d):= \{\run(w) \mid  w \in \dom(T) \wedge \height(w)=d\}\ .$$

We can finally define a run $\run$ of the \cta $\aut$ as \emph{accepting} when 
\begin{enumerate}
\item 
it is accepted by its underlying TA, and
\item
%$\cdet{\Delta}{\level(\run,d)}$ for all $d\in\nat$. 
% $\level(\run,d)$ is $\Delta$-color-deterministic for all $d\in\natz$. 
\yg{$\level(\run, d)$ has non-empty options for all $d\in\natz$.}
\end{enumerate}
The language $\langof \aut$ of $\aut$ is then the set of trees accepted
by~$\aut$. 

\yg{
\subsection{Alternative definition of CTA}
The $\Delta$-color-deterministic constraint above basically says which combinations of transitions are allowed. In particular, transitions of the same top are never allowed.\\
The definition of $\Delta$-color-deterministic makes this automata non-monotonic, i.e. the language set is not increase/decrease as the transition set increase/decreases, which makes minimization difficult.  Removing a transition will loosen the $\Delta$-color-deterministic constraints, it may turn some transition set from ``non-$\Delta$-color-det'' to ``$\Delta$-color-det'' and accept new trees.\\
An alternative definition is: First, take $\bigcap_{\delta\in\Gamma} \ell(\delta)$ as $Col'(\Gamma)$
and restrict $Col'(\level(\run,d))$ to be non-empty. Second, $\Delta$ must be disjointly colored, that is, for all $\delta_1\ne\delta_2\in\Delta$
\[
    top(\delta_1)=top(\delta_2)\implies\ell(\delta_1)\cap\ell(\delta_2)=\emptyset
\]
in this ``dual" definition, let's call it CTA', colors are treated as choices instead of constraints. A $\level(\run,d)$ is considered valid if it has non-empty choices and transitions of same top are invalid. In CTA', whether a run $\run:D\to\Delta$ is accepting is a function of transition used in that run $\{\run(x)|x\in D\}$, removing unused transition wouldn't change acceptance of existed runs, therefore it is monotonic.\\
It not surprising CTA and CTA' have same expressiveness, actually there is simple translation between them. Given a CTA', by relabeling each transitions with complement color, we get a equivalent CTA. Given a CTA with $N$ colors, we can first label each transition with a formula $\varphi(\delta)$ 
\[\varphi(\delta)=(\bigwedge_{i\in\ell(\delta)}x_i)\land(\bigwedge_{top(\delta')=top(\delta),\delta'\ne\delta}{\neg \bigwedge_{j\in\ell(\delta')} x_j}) \]
where $x_i$ indicates $i\in COL(\Gamma)$, then models for the formula can be use as choices of the transition, i.e. $\ell'(\delta)=\{m|m\models\varphi(\delta)\}$ is a labeling function for equivalent CTA' with at most $2^N$ color(choices).\\
The main drawback of CTA' is that we may need more color to encode non-deterministic choices. Fortunately, applying gate operations we explored to CTA', will not introduce new colors. The only scenario that CTA' introduce new color but CTA doesn't, is intersection.
}

%*******************************************************************************




%\hide{
%
%\paragraph{Emptiness Problem} 
%Given a CTA $\aut = \tuple{Q,\Sigma,\Delta,\rootstates,\ell}$. 
%Recall that for a non-leaf transition $\delta = \ctranstree {q}{f}{q_1,\dots,q_{\Arity(f)}}{C} \in \Delta$, we denote by $\mathtt{top}(\delta)=q$ and $\mathtt{bottom}(\delta) = \{ q_i \}_{i=1}^{\Arity(f)}$. 
%For a leaf transition $\delta = \ctranstree {q}{c}{}{C} \in \Delta_0$, we define $\mathtt{bottom}(\delta):= \{c\} \subset \Sigma_0$ for convenience. Now, let us form a \emph{directed graph} $G_\aut= (V,A)$ associated with a CTA $\aut$ as follows: 
%\begin{enumerate}[(i)]
%    \item the set $V$ of vertices corresponds to the set $2^{Q \cup \Sigma_0}$ of subsets $\mathtt{S} \subseteq Q \cup \Sigma_0$; 
%    \item there is an arrow $a=(\mathtt{S},\mathtt{T})\in A$ from a vertex $\mathtt{S}$ to a vertex $\mathtt{T}$ if and only if 
%    there exists a sequence of transitions $\{\delta^j\}_{j\in J}$, indexed by some set $J$, such that \begin{inparaenum}
%        \item $\{ \mathtt{top}(\delta^j) \mid j \in J \} = \mathtt{S}_Q := \mathtt{S} \cap Q$;
%        \item $\cup_{j \in J} \mathtt{bottom}(\delta^j) = \mathtt{T}$; and
%        \item for each $q \in \mathtt{S}_Q$ and each $\delta^j = \ctranstree {\mathtt{top}(\delta^j)} {f_j} {q_1,\dots,q_{\Arity(\delta^j)}}{C_j}$ with $\mathtt{top}(\delta^j)=q$, 
%        it holds that $|\{ \delta \mid \delta \in \Delta(q,f_j) \land \ell(\delta) \subset \cup_{j \in J} \ell(\delta^j) \}| \leq 1$; 
%        \item we remove all the isolated vertices. 
%    \end{inparaenum}
%\end{enumerate}
%Since $Q$ and $\Delta$ are finite sets by definition, the directed graph $G_\aut$ is finite. 
%A vertex $\mathtt{S} \in V$ is called a \emph{source} if $\mathtt{S} = \{q\}$ is a singleton set and $q \in \rootstates$. 
%A vertex $\mathtt{T} \in V$ is called a \emph{terminal} if $\mathtt{T} \subseteq \Sigma_0$. 
%
%Let $\run$ be a run over a tree $T$ accepted by the CTA $\aut$. We have by definition \begin{inparaenum}
%    \item $q = \mathtt{top}(\run(\epsilon)) \in \rootstates$ corresponds to a source vertex of $G_\aut$;
%    \item on each height $d>0$, we have $Q(\run,d)=\{ \mathtt{top}(\run(w)) \mid w \in \dom(T) \land |w|=d \}$ and let $\mathtt{S}_d:= \{ c \mid c \in \Sigma_0 \land \exists \delta = \transtree {q'}{c}{} \in \level(\run,d-1)  \} $, the set $Q(\run,d) \cup \mathtt{S}_d$ corresponds to a vertex of $G_\aut$;
%    \item the sequence of transitions $\level(\run,d)$ satisfies the color constraints \eqref{def:CTArun} and
%    $Q(\run,d+1) \cup \mathtt{S}_{d+1} =  \cup_{\delta \in \level(\run,d)}\mathtt{bottom}(\delta)$. Thus the family of transitions $\{\run(w) \mid w \in \dom(T) \land |w|=d \}$ corresponds to an arrow $a=(Q(\run,d-1)\cup \mathtt{S}_{d-1}, Q(\run,d) \cup \mathtt{S}_{d} ) \in A$;
%    \item and at the leaf nodes what we remain are the constant symbols, which corresponding to a terminal vertex of $G_\aut$.  
%\end{inparaenum} Thus an accepting run $\run$ corresponds to a path in $G_\aut$ from a source vertex to a terminal vertex. In other word, we reduce the following emptiness problem to the reachability problem from a source vertex to a terminal vertex in $G_\aut$.
%
%\noindent
%\textbf{Emptiness}
%
%\noindent
%\textbf{Instance} A CTA $\aut$
%
%\noindent
%\textbf{Answer} ``yes'' if and only if $\lang(\aut)$ is empty 
%\begin{theorem}
%    The emptiness problem of a given CTA $\aut$ is decidable. 
%\end{theorem}
%\begin{proof}
%    By the above discussion, the problem is reduced to the reachability problem of the corresponding directed graph $G_\aut$. The latter is decidable. 
%\end{proof}
%
%\paragraph{Inclusion Algorithm} In this paragraph we show that the inclusiveness of CTAs is decidable. 
%
%\noindent
%\underline{Input}: A CTA $\aut_S=\tuple{Q_S,\Sigma,\Delta_S,\rootstates_S,\ell_S}$, a CTA $\aut_R=\tuple{Q_R,\Sigma,\Delta_R,\rootstates_R,\ell_R}$.
%
%\noindent
%\underline{Output}: True if $\lang(\aut_S) \subseteq \lang(\aut_R)$, False otherwise. 
%
%Given two CTAs $\aut=\tuple{Q_\aut,\Sigma,\Delta_\aut,\rootstates_\aut,\ell_\aut}$ and $\autb=\tuple{Q_\autb,\Sigma,\Delta_\autb,\rootstates_\autb,\ell_\autb}$, 
%we are going to construct a directed graph $G_{\aut,\autb} = (V,A)$ inductively as follows: let $G_\aut=(V_\aut,A_\aut)$ and $G_\autb=(V_\autb, A_\autb)$ be the corresponding directed graphs defined as above. 
%Note that by the construction of the graph $G=(V,A)$ associated to a CTA, each arrow $a \in A$ corresponds to a sequence of color-consistent transitions, and we denote by $\underline{a}$ the sequence of its corresponding symbols. 
%\begin{enumerate}[(i)]
%    \item each vertex $x \in V$ corresponds to a tuple $(v_\aut, \mathtt{U}_\autb, \mathfrak{R})$ where \begin{inparaenum}
%        \item $v_\aut \in V_\aut$;
%        \item $\mathtt{U}_\autb \subset V_\autb$;
%        \item $\mathfrak{R} = (\mathfrak{R}_{v_\aut,v^i_\autb})_{v^i_{\autb} \in \mathtt{U}_\autb }$ is a collection of binary relations $\mathfrak{R}_{v_\aut,v^i_\autb}$, that is, when viewing $v_\aut$ and $v^i_\autb$ as subsets of $Q_\aut \cup \Sigma_0$ and $Q_\autb \cup \Sigma_0$ respectively, $\mathfrak{R}_{v_\aut,v^i_\autb}: v_\aut \times v^i_\autb  \to \{0,1\}$ is a Boolean function and satisfies that, for $x,y \in \Sigma_0$, $\mathfrak{R}_{v_\aut,v^i_\autb} (x,y) = 1$ if $x=y$ and $0$ otherwise. 
%%        indexed by elements $v^i_\autb \in \mathtt{U}_\autb$, over $v_\aut$ and $v^i_\autb$ by viewing vertices $v_\aut$ and $v^i_\autb$ as subsets of $Q_\aut \cup \Sigma_0$ and $Q_\autb \cup \Sigma_0$ respectively such that $\mathfrak{R}_{v_\aut,v^i_\autb}(x,y) = \delta_{x,y}$ for $x,y \in \Sigma_0$. 
%    \end{inparaenum}
%    \item there is an arrow $a=(x^1,x^2) \in A$ from a vertex $x^1=(v^1_\aut,\mathtt{U}^1_\autb,\mathfrak{R}^1)$ to another $x^2=(v^2_\aut,\mathtt{U}^2_\autb,\mathfrak{R}^2)$ if and only if \begin{inparaenum}
%        \item there exists an arrow $(v^1_\aut,v^2_\aut) \in A_\aut$ in $G_\aut$;
%        \item for each $v^{2,j}_\autb \in \mathtt{U}^2_\autb$ there exist a $v^{1,j}_\autb \in \mathtt{U}^1_\autb$ and an arrow $a^{j} = (v^{1,j}_\autb,v^{2,j}_\autb) \in A_\autb$ such that $\underline{a^j} = \underline{a}$ for all $j$;
%        \item $\mathfrak{R}^2$ is induced by $\mathfrak{R}^1$ together with $a^j$'s, i.e., $\mathfrak{R}^2_{v^2_\aut,v^{2,i}_\autb}(q^2_{\aut,p},q^{2,i}_{\autb,p}) = \mathfrak{R}^1_{v^1_\aut,v^{1,i}_\autb}(q^1_\aut,q^{1,i}_\autb)$ for all transitions 
%        $\ctranstree {q^1_\aut}{f}{q^2_{\aut,1},\dots,q^2_{\aut,\Arity(f)}}{C}$, 
%        $\ctranstree {q^{1,i}_\autb}{f}{q^{2,i}_{\autb,1},\dots,q^{2,i}_{\autb,\Arity(f)}}{C}$ corresponding to the arrow $a$ and $0$ otherwise.
%    \end{inparaenum}
%    \item we remove all the isolated vertices.
%\end{enumerate}
%We call a vertex $x \in V$ a \emph{source} of $G_{\aut,\autb}$ if $x$ is of the form $(\{q_\aut\},\{\{q^j_\autb \}\}_{q^j_\autb \in \rootstates_\autb},\mathfrak{R})$ where $\{q_\aut\}$ is a source of the graph $G_\aut$ and $\mathfrak{R}_{\{ q_\aut \},\{ q^j_\autb \} }(q_\aut,q^j_\autb) =1$ for all $j$. And a vertex $x=(v_\aut,\mathtt{U}_\autb,\mathfrak{R}) \in V$ is called a \emph{terminal} if and only if \begin{inparaenum}
%    \item $v_\aut$ is a terminal as a vertex in $G_\aut$;
%    \item there is at least a $v_\autb \in \mathtt{U}_\autb$ such that $v_\autb$ is a terminal in $G_\autb$ and $v_\autb = v_\aut$ viewed as subsets of $\Sigma_0$.
%\end{inparaenum}
%
%
%Similar to the discussion in the previous paragraph, for each accepting run $\run_\aut$ of $\aut$ over a tree $T$ there exists an accepting run $\run_\autb$ of $\autb$ over $T$ if and only if there exists a path in $G_{\aut,\autb}$ from a source vertex to a terminal vertex. Thus we reduce the inclusiveness of given two CTAs to the reachability problem in the associated directed graph. In other word, we have
%
%\begin{theorem}
%    The inclusiveness of given two CTAs is decidable.
%\end{theorem}
%\qed }

\hide{
\begin{theorem}
\ol{superseded by \cref{thm:cta_emptiness}? or give this as a practical algorithm?}
\yfc{it is superseded, but need to be careful about the notations used in the next theorem.}
  It is decidable whether the language of a given \cta is empty.
\end{theorem}
\begin{proof}
To decide whether the language of a \cta $\aut =
  \tuple{Q,\Sigma,\Delta,\rootstates}$ is empty, we build a directed graph
  $G_\aut= (V,A)$ associated with $\aut$ as follows. The set $V$ of
  \emph{vertices} consists of subsets of $Q$ where
\begin{enumerate}
\item
each $\{q\}$ with $q \in \rootstates$ is a \emph{source} vertex and
\item
the empty set $\emptyset$ is the \emph{terminal} vertex.
\end{enumerate}
The graph has an arrow $a=(\mathtt{U},\mathtt{V})\in A$ from a vertex $\mathtt{U}$ to a vertex $\mathtt{V}$ if and only if $\mathtt{V}$ is constructed from $\mathtt{U}$ by
    \begin{enumerate}
            \item choosing one transition from  $\Delta(q)$ per $q\in \mathtt{U}$ 
into a $\Delta$-color-deterministic set $J$ (note that the choice of the set $J$ is not unique, hence $\mathtt{U}$ can have multiple outgoing arrows), and
            \item taking $\mathtt{V}$ as the set of bottom states of the transitions in $J$. 
    \end{enumerate}
Since $Q$ is a finite set by definition, the directed graph $G_\aut$ is finite, and  
it holds that $\lang(\aut)=\emptyset$ iff the terminal vertex cannot be reached from a source vertex in it.
\end{proof}}
